Game-Theoretic Energy Source Allocation Mechanism in Smart-Grids

This work studies the decentralized and uncoordinated energy source selection problem for smart-grid consumers with heterogeneous energy profiles and risk attitudes: they compete for a limited amount of renewable energy in their local community, at the risk of paying a higher cost if that energy is not enough to supply all such demand. We model this problem as a non-cooperative game and study the existence of mixed-strategy Nash equilibria (NE) under the proportional allocation policy employed when the total demand for renewable energy exceeds the available one. We derive under NE closed-form expressions for the resulting total renewable energy demand and social cost under varying consumer profiles, energy costs and availability. The analysis also provides useful guidelines as to what consumers should do (compete or not) based on their risk attitude or if they should be more risk-taking, under certain conditions. Finally, we study numerically the efficiency of this decentralized scheme compared to a centralized one via the price-of-anarchy metric.

==> algorithms.tex <==
\section{Algorithm} \label{sec:algorithms}

In Section \ref{sec:uncoordinated_extra_demand}, we studied theoretically the distributed and uncoordinated energy selection problem of consumers, i.e., we provided analytical formulations of the dominant- and mixed-strategy NE in different cases. In this section, we design a distributed, uncoordinated algorithm that leads to mixed-strategies NE and in cases where there exists no clear dominant-strategy for all consumers (i.e., Cases $2(a)$, $2(c)$, and $4$). Indeed, in the presence of dominant strategies (i.e. Cases $1$, $2(b)$, and $3$), the decisions of each player are independent on the other players' decisions and can be computed directly. The developed iterative algorithm is based on a best response scheme. The proposed algorithm accounts for both energy
source allocation policies, namely PA and ES. Most importantly, the
algorithm is distributed and requires minimum information exchange
between the consumers. In particular, there is no need
for a central operator to run it or for direct communication
channels between consumers.


As previously mentioned, all consumers with a certain type share the same strategy. Consequently, at a given iteration, the proposed algorithm sequentially computes the best strategy of each consumers' type and then applies it to all consumers that share this type (line \ref{line:retrievestrategy}). In the initialization step, all consumers' types are ordered at random in a list denoted $\Sigma$, which represents the order in which the consumers' types will play at each iteration (lines \ref{line:sigma1}-\ref{line:sigma4}). And the value of the vector $EQT$, which represents if each consumers' type has played at a given iteration is initialized to $\bm{0_M}$ at the beginning of each new outer iteration.

%%%
At a given outer iteration, all the consumers' types play one after the other to update their probability $p_{RES,\vartheta_i}^{x,*}$, which represents their best response to the strategies that have been already been chosen by the other consumers' types. The vector of NE probability distribution for all consumers denoted $EQP$ is updated after their turn, and $EQT(\vartheta_i) \gets 1$, denoting that this consumers' type has played.

%%
As we aim to minimize information exchange, the strategies that have already been chosen by the other consumers' types are not known. Instead the consumers update a common variable $X_\Sigma$, which encodes that information as an aggregate amount. For the PA policy, the aggregate quantity $X_\Sigma$ represents the total average energy competing for $RES$ up to the current iteration. For the ES policy, it represents the total average number of consumers competing for $RES$ up to the current iteration. This can be seen by comparing Eqs. \eqref{eq:prop_alloc_energy}, \eqref{eq:eq_sharing_energy} with lines \ref{line:PAconstr} and \ref{line:ESconstr} of the algorithm correspondingly. 
%%%
Based on the value of the aggregate vector $X_\Sigma$ in their turn, each consumers type $\vartheta_i$ computes their best response by minimizing their expected cost of energy (line \ref{line:bestresponse}), which is given by
\begin{align}
    cost(p_{RES,\vartheta_i}^{x}) & = p_{RES,\vartheta_i}^{x}\big[rse_{\vartheta_i}^x(\mathbf{n_i})c_{RES}+(E_{\vartheta_i}-rse_{\vartheta_i}^x(\mathbf{n_i})) \nonumber \\ 
    & \cdot\gamma \cdot c_{RES}\big]
    + (1-p_{RES,\vartheta_i}^{x})\epsilon_{\vartheta_i}\cdot E_{\vartheta_i}\cdot \beta \cdot c_{RES}. \label{eq:personalcost}
\end{align}

One limitation of the best response is that the first consumers type chosen at random, i.e. $X_0$ has a great advantage, since they choose as much RES as they want. In order to eliminate this effect, we introduce a capping system at each iteration, which enforces that the best response competing probability $p_{RES,\vartheta_i}^{x,*}$ computed in line \ref{line:bestresponse} is multiplied with a random number drawn from a uniform distribution $rand \sim \mathcal{U}(0,1)$, such that:
\begin{align}\label{eq:cap}
    f_{cap}^{rand}(p_{RES,\vartheta_i}^{x,*}) &= rand \cdot p_{RES,\vartheta_i}^{x,*}.
\end{align}

As a result, after one external iteration (line \ref{line:external_round}), in which all consumers' types have played once, there may still exist available RES non-allocated. If this happens, the algorithm will require additional iterations, in which all consumers' types update their strategies, to to reach an equilibrium state (line \ref{line:probincrease}). In practice the algorithm continues until one of the two following conditions hold: (i) equilibrium is reached, which means that the players do not wish to change their actions unilaterally, with respect to the previous iteration (line \ref{line:equilibrium}), or (ii) a maximum number of external iterations ($N_{iter}$) is reached. The steps of this algorithm are summarized in Algorithm \ref{algorithm} below.

%The two methods can produce significantly different results, because the implementation of an \emph{equal cap} results to very similar values of equilibrium probabilities for all consumer types, while the \emph{random cap} can produce any solution on the equilibrium hyperplane.


%For example, assume a game with two types, type $0$ and $1$, with both competing probabilities initialized to $0$. Let the first consumer to play be of type $0$. The player calculates their best strategy, let that be $p_{RES,0}^{(1)}$ and then updates $X_\Sigma$ accordingly. Then, a player with type $1$ takes turn, calculates their best response $p_{RES,1}^{(1)}$ and updates $X_\Sigma$. Now is the turn of a type $0$ player, who has the encoded information in $X_\Sigma$. The player calculates their best response, namely $p_{RES,0}^{(2)}$. However, since $X_\Sigma$ is linear with respect to the competing probabilities (see Algorithm \ref{algo}), the current state of the game is equivalent to $(p_{RES,0}, p_{RES,1}) = \left(p_{RES,0}^{(1)}+p_{RES,0}^{(2)}, p_{RES,1}^{(1)}\right)$. In particular, when each consumer is playing, they incrementally increase the shared strategy of their type, which is stored in variable $Compt\_info$, by the optimal amount. The algorithm ends, when the change in competing probabilities is less than the predefined convergence tolerance or if it reaches the maximum number or rounds, namely $N_{iter}$.

%Since there is no distinction between players of the same type, all consumers of the same type share the same expected cost.

\begin{small}
\begin{algorithm}[h!] \label{algorithm}
    \SetAlgoLined
    \textbf{Input} $x$: Equal to PA or ES depending on the energy allocation policy; $N_{iter}$\\
    \textbf{Output} $EQP$: Vector of NE probability distributions for each consumer type; \\\
    \textbf{Initialization: \label{line:init}}\\
    $(p^{x}_{RES,\vartheta_i}, p^{x}_{nonRES,\vartheta_i}) \gets (0,1), \forall \vartheta_i  \in \vartheta$ \;
    If Case 2(a): $X_\Sigma \gets 0$, $\Sigma \gets$ all consumers types \label{line:sigma1}\;
    If Case 2(c): $X_\Sigma \gets 0$, $\Sigma \gets$ all consumers types in $\Sigma_2$ \label{line:sigma2}\; 
    If Case 4 $\&$ $x=PA$: $X_\Sigma \gets \sum_{ \vartheta_j \in \Sigma_1 \setminus \{ \vartheta_i \} } r_{\vartheta_j} (N-1)E_{\vartheta_j}$, $\Sigma \gets$ all consumers in $\Sigma_2$ \label{line:sigma3}\; 
    If Case 4 $\&$ $x=ES$: $X_\Sigma \gets \sum_{ \vartheta_j \in \Sigma_1 \setminus \{\vartheta_i\} } r_{\vartheta_j} (N-1)$, $\Sigma \gets$ all consumers in $\Sigma_2$ \label{line:sigma4}\;
    $EQT \gets \mathbf{0}_M$, $EQP \gets \mathbf{p}^{x}$\;
    \For{$iter \gets 1$ \KwTo $N_{iter}$ \label{line:external_round}}{
        $EQT \gets \mathbf{0}_M$\;
        $EQP_{old} \gets EQP$\;
        \For{each consumers' type $\vartheta_i \in \Sigma$}{
            \If{$EQT(\vartheta_i) = 1$}{
            Consumer $i$ retrieves $p_{RES,\vartheta_i}^x$ from $EQP(\vartheta_i)$\; \label{line:retrievestrategy}}
            \Else{
                \uIf{$x=PA$}{
               $rse_{\vartheta_i}^{PA}(p_{RES,\vartheta_i}^{PA})=\frac{E_{\vartheta_i}\cdot \mathcal{ER}}{X_\Sigma +(N-1) r_{\vartheta_i} p^{PA}_{RES, \vartheta_i} E_{\vartheta_i} + E_{\vartheta_i}}$\label{line:PAconstr}\;}
                \ElseIf{$x=ES$}{ $rse_{\vartheta_i}^{ES}(p_{RES,\vartheta_i}^{PA})=\frac{\mathcal{ER}}{X_\Sigma +(N-1) r_{\vartheta_i} p^{PA}_{RES, \vartheta_i} + 1}$\label{line:ESconstr} \;}
                $p_{RES,\vartheta_i}^{x,*}\gets \,\underset{p_{RES,\vartheta_i}^x} {\mathrm{arg\,min}}\, cost(p_{RES,\vartheta_i}^x)$\label{line:bestresponse}, from Eq. \eqref{eq:personalcost}\;
                $p_{RES,\vartheta_i}^{x,cap}\gets f_{cap}(p_{RES,\vartheta_i}^{x,*})$, from Eq. \eqref{eq:cap}\;
                $EQT(\vartheta_i) \gets 1$, \\$EQP(\vartheta_i) \gets \,EQP(\vartheta_i)+p_{RES,\vartheta_i}^{x,cap}$\label{line:probincrease}\;
                \uIf{$x=PA$}{
                    $X_\Sigma \gets \,+ (N-1)r_{\vartheta_i}p_{RES,\vartheta_i}^{x,cap}E_{\vartheta_i}$\;}
                \ElseIf{$x=ES$}{
                    $X_\Sigma \gets \,+ (N-1)r_{\vartheta_i}p_{RES,\vartheta_i}^{x,cap}$\;}
                }
            }\If{$EQP\equiv EQP_{old}$ \label{line:equilibrium}}{
                Exit\;
        }
    }
    \caption{Distributed algorithm for uncoordinated NE.}
\end{algorithm}
\end{small}

With respect to privacy, the designed distributed uncoordinated mechanism does not require the exchange of sensitive information among users. If the number of consumers $N$ is much higher than the number of energy demand profiles $M$, inferring the consumers' energy profiles is difficult. In addition, further privacy concerns can be handled by encrypting the outcomes $EQT$ and $EQP$ of the algorithm at each iteration and appropriately authenticating users. Such an encryption could ensure that a consumer is able to read only information with respect to its own profile. However, if the second in row computing consumers' type has the same profile as the first one, the profile of the first consumers' type is revealed. To avoid this, the first consumers' type could choose a set of profiles including its own and impose that the second consumer does not have a profile in this set. This can easily be achieved if the number of consumers' types is sufficient, which is a realistic assumption. In the special case where $N=M$, communicating the outcomes $EQT$ and $EQP$ is not needed; the computing consumer should only know the current value of $X_\Sigma$. 
 
%The optimization problem solved in lines \ref{line:min1}-\ref{line:min2} is a best response one, similarly to the algorithms of \cite{jacquot18}. In addition, in lines \ref{line:PAconstr} and \ref{line:ESconstr}, the algorithm imposes constraints in order to compute probabilities that satisfy the necessary conditions for NE, as obtained by the analysis in Section \ref{sec:uncoordinated_extra_demand}. In line \ref{line:randomization}, we introduce randomization in the choice of $p^{x, *}_{RES, \vartheta_i} $, in order to avoid providing all the chances of competing for RES to the first in row examined consumer profiles. Due to this randomization, in order to ensure efficiency, i.e., competing for all the available RES, we introduce a second loop of iterations (line \ref{line:whileloop}) that terminates when the computed probabilities $Compt\_info\{2\}$ do not change from the previous iteration. Randomization stops after $MI$ iterations, so as to increase the chances that the external iterations (line \ref{line:whileloop}) will terminate. The chances increase due to our assumption that the users' aggregate demand exceeds the RSE capacity (Section \ref{sec:uncoordinated_extra_demand}).

%\begin{proposition}The algorithm terminates at a NE at a maximum of $N_{iter}+2$ external iterations. 
%\end{proposition}
%\begin{proof} In the cases where the algorithm applies consumers aim to opt for RES, each with the maximum possible probability in $[0,1]$. As a result, due to the constraints in lines \ref{line:PAconstr} and \ref{line:ESconstr}, at $iter^*$ at most equal to $MI+1$, the Eq. \eqref{eq:probrelation} or \eqref{eq:probrelationes} (depending on $x$) will be satisfied by the mixed strategies chosen by the algorithm or the mixed strategies will take the closest possible values to those satisfying \eqref{eq:probrelation} or \eqref{eq:probrelationes} due to their projection in $[0,1]$ (line \ref{line:projection}). According to the analysis in Section \ref{sec:uncoordinated_extra_demand}, these probabilities are NE. Due to the constraints imposed by the algorithm, at iteration $iter^*+1$, (obviously, at most equal to $MI+2$), the probabilities in $Compt\_info\{2\}$ cannot change; thus, it will be set $no\_exit=False$ and the algorithm will terminate at a NE. The termination of the algorithm might not happen in an earlier external iteration due to the randomization of line \ref{line:randomization}.
%\end{proof}

Finally, this algorithm schedules consumers' loads in day and night zones once, in the beginning of the day zone. However, it can be repeated several times in a non-real time scale e.g., in an intra-day time scale (e.g., every 1 h during the day zone) in a Model Predictive Control fashion, where at each repetition (i) the consumers reconsider their energy demand profiles by subtracting the loads that have been already served, (ii) the forecast of the RES, $\mathcal{ER}$ is updated. 

==> coordinated.tex <==
\section{Centralized Coordinated energy source allocation}\label{sec:coordinated}

In this section, we study a centralized mechanism that coordinates how consumers' demand will be served (i.e., by which source) in order to minimize the social cost (i.e., Eqs. \eqref{eq:social_cost_pa_extra_demand} for proportional allocation and Eqs. \eqref{eq:social_cost_es} for equal sharing). Furthermore, we evaluate the side-effects that stem from the distributed, uncoordinated energy source selection as far as the social welfare is concerned via the Price of Anarchy (PoA) measure \cite{Koutsoupias09}. PoA is expressed as the ratio of the social cost in the worst-case equilibria over the optimal-minimum social cost of the centralized mechanism.
We study the PA mechanism analytically in most of the distinguished cases. For the ES mechanism, the centralized decisions for minimizing the social cost are harder to derive analytically and we will present numerical evaluations in Section \ref{sec:eval} using a software optimization tool such as Mathematica or MATLAB. The same is true for the PoA, which can be obtained as indicated in Section \ref{sec:poa}. %may be alleviated with control mechanisms that coordinate individual decisions towards more socially
%efficient choices. In the sequel, we describe two approaches that differ on the required infrastructure and the amount of control they impose upon the energy source allocation. Furthermore, the (in)efficiency of the equilibria action profiles as derived in Section \ref{sec:uncoordinated_extra_demand}, %Sections \ref{sec:uncoordinated_no_extra_demand} and \ref{sec:uncoordinated_extra_demand}, 
%resulting from the strategically selfish individual
%decisions, is assessed through the broadly used metric of the Price of Anarchy (\textit{PoA}) \cite{Koutsoupias09}. This metric
%expresses the ratio of the social cost in the worst-case equilibria over the optimal-minimum social cost as derived under the two coordination approaches.
%
%%\subsection{Centralized Coordination Mechanisms}\label{sec:opt_central_no_extra_demand}
%
%The side-effects in energy pursuit may be eliminated by introducing centralized mechanisms
%that undertake both the information processing and the decision-making tasks. These mechanisms coordinate the service of consumers' demand to ensure the optimal utilization of RES.%, on the one side, and the elimination of the congestion penalty, on the other side (Ref. Section \ref{sec:game}).

\subsubsection{Proportional Allocation}\label{sec:opt_pa_central_no_extra_demand}
 Let $p^{PA,OPT}_{RES,\theta_i} (p^{PA,OPT}_{nonRES,\theta_i})$ stand for the probability that users of energy profile $\theta_i \in \Theta$ opt (do not opt) for RES, as decided by the centralized coordinated mechanism, under the proportional allocation. $\mathbf{p^{PA,OPT}}$ is defined similarly to $\mathbf{p^{PA,NE}}$. The following cases are distinguished.

It is important to note that the centralized coordination mechanism will achieve a demand for RES equal to $D^{PA,OPT}=min(\sum_{\theta_j \in \Theta}r_{\theta_j}NE_{\theta_j},\mathcal{ER})$, in all considered cases. 

\textbf{Case $1$.} The RES capacity exceeds the aggregated consumer demand. Then, all consumers (for both cases of risk-seeking and risk-conservative) are directed to the RES and $p^{PA,OPT}_{RES,\theta_i}=1$, $\forall \theta_i \in \Theta$.

In all the rest cases, the aggregated consumer demand exceeds the RES capacity. 

\textbf{Case $2$.} The risk-aversion degrees satisfy $\epsilon_{\vartheta_i}=\epsilon'<\gamma/\beta$, $\forall i\in \mathcal{N}$. This case includes the risk-seeking consumers ($\gamma/\beta>1$). Then, $p^{PA,OPT}_{RES,\theta_i}$, for all  $\theta_i \in \Theta$ are chosen to match the RES demand to supply, that is, %$rNp^{PA,OPT}_{nonRES,0}E_0+(1-r)N p^{PA,OPT}_{nonRES,1}E_1=\mathcal{ER} $.

\vspace{-5pt}
\small
\begin{equation}
N \sum_{\theta_j \in \Theta}r_{\theta_j} E_{\theta_j}p^{PA,OPT}_{RES,\theta_j}=\mathcal{ER}.
\label{eq:optimal}
\end{equation}
\normalsize

The competing probabilities, $p^{PA,OPT}_{RES,\theta_i} $, lie in the range below, under the constraint of \eqref{eq:optimal},

\vspace{-5pt}
\footnotesize
\begin{align}
 \hspace{-5pt} 
 \Biggl[max\left\{0,\frac{\left[\mathcal{ER} -\sum_{\theta_j\neq \theta_i, \theta_j \in \Theta}r_{\theta_j}N E_{\theta_j}\right]}{r_{\theta_i}N E_{\theta_i}}\right\},
   %\notag\\
    % min\left(1,\mathcal{ER} \frac{1}{rNE_0}\right)
    min\left\{1,\frac{\mathcal{ER}}{r_{\theta_i}N E_{\theta_i}}\right\}
    \Biggr].
    \label{eq:prop_alloc_opt_bounds_0}
\end{align}
\normalsize


The cost due to the demand at night-rate is constant and equal to 
$\epsilon' N \sum_{\theta_j \in \Theta}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j} c_{noRES,N}=\epsilon'  ( N\sum_{\theta_j \in \Theta}r_{\theta_j}E_{\theta_j}- \mathcal{ER}) c_{noRES,N}$.

\textbf{Case $3$.} The different energy profiles are coupled with different degrees of risk-aversion, %, which is less than $\gamma/\beta$, %depart in their policy in adjusting their demand level to the estimated risk of an action, 
\ie $\exists$  $i,j\in \mathcal{N}: \gamma/\beta>\epsilon_{\vartheta_i} > \epsilon_{\vartheta_j}$. In this case, the night-rate social cost to be minimized is $Nc_{noRES,N} \sum_{\theta_j \in \Theta}\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j} $. The solution can be derived by a software optimization tool such as Mathematica or MATLAB. In addition, due to the fact that the RES demand should match its supply as in Case $2$,  the probabilities, $p^{PA,OPT}_{RES,\theta_i} $, lie in the ranges given in (\ref{eq:prop_alloc_opt_bounds_0}). 


%Therefore, it is minimized when consumers with energy profiles $\theta_j \in \Theta$, corresponding to higher values of $\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}$ are assigned lower values of $p^{PA,OPT}_{nonRES,\theta_j} $ and thus higher values of $p^{PA,OPT}_{RES,\theta_j} $ (i.e., they are prioritized for RES). In addition, due to the fact that the RES demand should match its supply as in Case $2$,  the probabilities lie in the ranges given in (\ref{eq:prop_alloc_opt_bounds_0}). 

To illustrate this result in a simple scenario, let us assume the case of two energy profiles and let us examine the expected cost at night-rate; $(\epsilon_0 r_0 N p^{PA,OPT}_{nonRES,0}E_0+\epsilon_1 r_1 N p^{PA,OPT}_{nonRES,1} E_1) c_{nonRES,N}$. Let us assume that $\epsilon_0> \epsilon_1$, then we can write $\epsilon_0= \epsilon_0'+\epsilon_1$, with $\epsilon_0'>0$. Thus, the expected cost at night-rate becomes $(\epsilon_0' r_0N p^{PA,OPT}_{nonRES,0}E_0+\epsilon_1 (r_0 N E_0+r_1 N E_1- \mathcal{ER}) ) c_{nonRES,N}$. The only controllable term is $\epsilon_0' r_0 N p^{PA,OPT}_{nonRES,0}E_0$ that is minimized when $ p^{PA,OPT}_{nonRES,0}$ is minimized, i.e., when its complementary $ p^{PA,OPT}_{RES,0}$ is maximized. Note that the expected cost due to use of RES will be always equal to $c_{RES} \mathcal{ER}$.

\textbf{Case $4$.} The risk-aversion degrees satisfy $\epsilon_{\vartheta_i} \geq \gamma/\beta$, $\forall i\in \mathcal{N}$. Then, the optimal centralized coordination mechanism would direct all consumers to RES, \ie $p^{PA,OPT}_{RES,\theta_i}=1$. This derives similarly to Case $3$ of Section \ref{sec:prop_alloc_eq_extra_demand}.
 
\textbf{Case $5$.} In this case, there exist two distinct sets of consumers' profiles $\Sigma_1$, $\Sigma_2$ with $\Sigma_1 \cap \Sigma_2= \emptyset$ and it holds that $\Biggl\{\epsilon_{\vartheta_i} \geq \gamma/\beta,~ \forall \vartheta_i \in \Sigma_1\Biggr\}$, and $\Biggl\{\epsilon_{\vartheta_i} < \gamma/\beta, ~ \forall \vartheta_i \in \Sigma_2\Biggr\}$. Then, it is dominant strategy for all consumers with energy profiles in the set $\Sigma_1$ to compete for RES, while the probability that consumers with energy profiles in the set $\Sigma_2$ compete for RES is shaped to totally utilize the remaining RES, i.e.,
%$[r+(1-2r)\vartheta_i]NE_{\vartheta_i}+[r+(1-2r)\vartheta_j]NE_{\vartheta_j}p^{PA,OPT}_{RES,\vartheta_j}=\mathcal{ER}$.

\vspace{-5pt}
\footnotesize
\begin{align}
&p^{PA,OPT}_{RES,\vartheta_i}=1, \forall \vartheta_i \in \Sigma_1; \notag \\
&p^{PA,OPT}_{RES,\vartheta_i}\in \nonumber \\
&\Biggl[\max\left\{0,\frac{\mathcal{ER}-\sum_{\theta_i \neq \theta_j, \theta_j \in \Theta}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}, \nonumber \\ & \min\left\{1,\frac{\mathcal{ER}-\sum_{ \theta_j \in \Sigma_1}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}  \Biggr],~ \forall \vartheta_i \in \Sigma_2.
\label{eq:prop_alloc_opt_p_cond}
\end{align}
\normalsize

Note that the probabilities of $\Sigma_2$ should be chosen under Eq. \eqref{eq:optimal}. However, the probability assignment to the energy profiles in the set $\Sigma_2$ for minimizing the social cost (i.e., equivalently the night rate cost because the demand in the day will be equal to $\mathcal{ER}$) should be done with the help of a software optimization tool. An exception is the case where $|\Sigma_2|=1$. In this special case, for $\vartheta_i \in \Sigma_2$, $p^{PA,OPT}_{RES,\vartheta_i}=\max\left\{0, \min\left\{1,\frac{\mathcal{ER}-\sum_{ \theta_j \in \Sigma_1}r_{\theta_j}N E_{\theta_j}}{r_{\theta_i}N E_{\theta_i}}\right\}\right\}$.


\textbf{Social Cost:} It is given as follows.

\begin{small}
\begin{align}
&C^{PA,OPT}(\mathbf{p^{PA,OPT}})= D^{PA,OPT} c_{RES}  \nonumber \\ 
&+Nc_{noRES,N} \sum_{\theta_j \in \Theta}\epsilon_{\theta_j}r_{\theta_j}E_{\theta_j}p^{PA,OPT}_{nonRES,\theta_j}.
 \label{eq:social_cost_pa_op1t}
 \end{align}
\end{small}


In the special case of risk-seeking consumers the social cost has a constant value with respect to the decision probabilities:
\begin{small}
\begin{align}
&C^{PA,OPT}= D^{PA,OPT} c_{RES}  \nonumber \\ 
&+ c_{noRES,N} \Biggl[ N\sum_{\theta_j \in \Theta} r_{\theta_j}E_{\theta_j}- D^{PA,OPT} \Biggr].
 \label{eq:social_cost_pa_opt2}
 \end{align}
\end{small}


\subsubsection{Price of Anarchy:} \label{sec:poa}
The (in)efficiency of equilibrium strategies is quantified by the Price of Anarchy (PoA). In order to compute the PoA for each particular case (where cases are distinguished with respect to the risk-aversion degree values and energy consumption values), we should compute the mixed strategy equilibrium that leads to the worst social cost for this case. PoA is computed as follows: %with respect to the consumers behavior (e.g., risk-seeking and risk-conservative), risk-aversion degree values and energy consumption values $E_0$, $E_1$.

\vspace{-5pt}
\small
\begin{align}
 \hspace{-5pt} \textit{PoA}^{PA}  = \frac{C^{PA,NE}_w}{C^{PA,OPT}(\mathbf{p^{PA,OPT}})},
\label{eq:poa_pa}
\end{align}
\normalsize
where the $C^{PA,NE}_w$ is the worst case social cost of the distributed, uncoordinated mechanism for the case of interest. Note that $C^{PA,OPT}(\mathbf{p^{PA,OPT}})$ is uniquely determined for each particular case.

In order to obtain $C^{PA,NE}_w$, we can solve a simple optimization problem to minimize the social cost $C^{PA,NE}(\mathbf{p^{PA,NE}})$ with respect to $\mathbf{p^{PA,NE}}$ (when there are multiple possible NE e.g., cases 2(a), 2(b) and 4 and subject to the corresponding probability constraints using a software optimization tool. Importantly, for the uncoordinated energy selection under PA, minimizing $C^{PA,NE}(\mathbf{p^{PA,NE}})$  is equivalent to minimizing the night-zone cost. The last observation is due to the fact that the demand $D^{PA,NE}$ is constant with respect to $\mathbf{p^{PA,NE}}$. 

In the special case of the risk-seeking consumers, from Eq. \eqref{eq:social_cost_pa_sc}, the social cost is constant with respect to the probabilities $\mathbf{p^{PA,NE}}$ for each case of energy profile values. In this case, $C^{PA,NE}_w$ is given by Eq. \eqref{eq:social_cost_pa_sc}.

For the risk-conservative consumers, assume the simple case of two energy profiles. Then, in all cases except subcase 2(a), the social cost is uniquely determined giving directly the value of $C^{PA,NE}_w$. For subcase 2(a)  the multiple combinations of probabilities can lead to NE with possibly different social cost values. Under the conditions of subcase (a), we can show that $\epsilon_1>\epsilon_0$. Thus, in this case the social cost is decreasing with $p_{RES,1}^{PA,NE}$  more than with $p_{RES,0}^{PA,NE}$, and its worst case value, $C^{PA,NE}_w$, is obtained using the maximum value of $p_{RES,0}^{PA,NE}$ and minimum of $p_{RES,1}^{PA,NE}$ from the range in Eq. \eqref{eq:prop_alloc_pa_bounds_0_extra_demand}.

For the ES allocation, $\textit{PoA}^{ES}$ is defined in a similar way with $\textit{PoA}^{PA}$ and we study it numerically in Section \ref{sec:eval}.
%\subsubsection{Equal Sharing}\label{sec:opt_es_central_no_extra_demand}
%In this section, we examine the decisions of a centralized coordination mechanism for the probabilities that users of each energy profile will opt for RES, denoted as $p^{ES,OPT}_{RES,\theta_i}$, $\theta_i \in \Theta$, under equal sharing.
%
%%Under an ideal optimal centralized coordination mechanism that equally allocates the available RES capacity to competing consumers, the derivation of the associated competing probabilities $p^{ES,OPT}_{RES,0}$ and $p^{ES,OPT}_{RES,1}$ factors in two distinct cases: (a) $E_0=E_1=E$ and (b) $E_0 <  E_1$. In the first case, 
%If $E_0=E_1=E$ the two renewable energy allocation policies are equivalent and therefore, the decisions of the centralized mechanism are the same as those in Section \ref{sec:opt_pa_central_no_extra_demand}. 
%
%Differently, if $E_0 <  E_1$ we distinguish the following cases: %the centrally computed probabilities that optimize the social cost (Ref. eq. (\ref{eq:social_cost_es_extra_demand})) are described by Table \ref{tb:opt_es_extra}.
%
%
%%\begin{table}[]
%%\centering
%%\caption{Probabilities under centralized coordination and equal sharing.}
%%\footnotesize
%%\label{tb:opt_es_extra}
%%\begin{tabular}{lcl}
%% $p^{ES,OPT}_{RES,0}$ \hspace{150pt}  $p^{ES,OPT}_{RES,1}$\\ \hline
%%  0 \hspace{165pt}   $min\left(1, \frac{\mathcal{ER}}{(1-r)NE_1}\right) $ \\ 
%% $min\left(1, \frac{\mathcal{ER}}{rNE_0}\right) $ \hspace{145pt}   0\\ 
%% 1 \hspace{70pt}   $min\left(1,max\left(0,\frac{1}{(1-r)}\left[\sqrt{\frac{\mathcal{ER}r(\gamma-1)}{E_1N(\gamma-\epsilon_1\beta)}} - r\right] \right)\right)$\\
%% 1 \hspace{105pt}  $min\left(1,max\left(0, \frac{1}{(1-r)}\left(\frac{\mathcal{ER}}{E_0N}-r\right)\right)\right)$\\
%% $min\left(1,max\left(0, \frac{1}{rN}\left[\frac{\mathcal{ER}}{E_1}-(1-r)N\right]\right)\right)$ \hspace{50pt}   1\\  
%%  $min\left(1,max\left(0, \frac{1}{rN}\left[\frac{\mathcal{ER}}{E_0}-(1-r)N\right]\right)\right)$ \hspace{50pt}   1\\  
%%\end{tabular}
%%\vspace{-5pt}
%%\end{table}
%%\normalsize
%
%
%\textbf{Case $1$.} The RES capacity exceeds the aggregated consumer demand. Then, all consumers (for both cases of risk-seeking and risk-conservative) are directed to the RES and $p^{ES,OPT}_{RES,\theta_i}=1$, $\forall~\theta_i \in \Theta$.
%
%\textbf{Case $2$.} Each one of the quantities $rN E_0$ and $(1-r) N E_1$ exceed the RES capacity. Then, (i) if $\epsilon_i \geq \frac{\gamma}{\beta}, \forall i \in \mathcal{N}$, $p^{ES,OPT}_{RES,0}=1$, $p^{ES,OPT}_{RES,1}=1$ (shown as in Case $3$, Section \ref{sec:prop_alloc_eq_extra_demand}) and (ii) if $\gamma> min(\epsilon_0\beta, \epsilon_1\beta)$ then all consumers competing for RES should have the same energy profile. Thus, the renewable energy will not remain unused due to the equal sharing allocation. % (by providing energy shares that exceed low-to-moderate energy demand, $E_0$) while consumers incur congestion penalties (by providing energy shares not sufficient to respond to their energy demand).
%For case (ii), the centralized coordination mechanism allocates the RES exclusively to consumers of energy profile, $\vartheta_i$, coupled with the highest risk-aversion degree, i.e., $\epsilon_{\vartheta_i}>\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. This is shown in a similar way as in Case $3$ of Section \ref{sec:opt_pa_central_no_extra_demand} and considering that the demand for RES will be equal to $\mathcal{ER}$ and will be equal to the aggregate of the allocated RES to all consumers.%, namely, to consumers with the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$.
% For instance, if $\epsilon_0\geq\epsilon_1$ the competing probabilities under optimal allocation are $p^{ES,OPT}_{RES,1}=0$ and $p^{ES,OPT}_{RES,0}=min\left(1, \frac{\mathcal{ER}}{rNE_0}\right)$, if $\gamma >\epsilon_0\beta$, or $p^{ES,OPT}_{RES,0}=1$, otherwise. Similarly, if $\epsilon_1\geq\epsilon_0$ the competing probabilities under optimal allocation are $p^{ES,OPT}_{RES,0}=0$ and $p^{ES,OPT}_{RES,1}<min\left(1, \frac{\mathcal{ER}}{(1-r)NE_1}\right) $, if $\gamma > \epsilon_1\beta$, or $p^{ES,OPT}_{RES,1}=1$, otherwise.
%
%\textbf{Case $3$.} Each one of the quantities $rN E_0$ and $(1-r) N E_1$ by itself does not exceed the RES capacity. Then, if also $\epsilon_i \geq \frac{\gamma}{\beta}, \forall i \in \mathcal{N}$, then $p^{ES,OPT}_{RES,0}=1$, $p^{ES,OPT}_{RES,1}=1$ (shown as in Case $3$, Section \ref{sec:prop_alloc_eq_extra_demand}). However, the under other conditions, the solution is more complicated and can be derived by a tool such as Mathematica or MATLAB.
%
%%Under lower aggregate demand levels, the coordination mechanism allows serving with RES heterogeneous energy consumption profiles, taking into consideration first the degree of risk-aversion of the two classes of consumers  and second the aggregate demand shaped by each class. The resulting competing probabilities are drawn from Table \ref{tb:opt_es_extra}, starting from $p^{ES,OPT}_{RES,0}=p^{ES,OPT}_{RES,1}=1$ for low aggregate demand and converging to the previously cited values when both the aggregate demands shaped by low-to-moderate and high energy consumers exceed the RES capacity.
%
%The Price of Anarchy derives in a similar fashion as in Section \ref{sec:opt_pa_central_no_extra_demand} and we omit the details due to lack of space. Notice that for the uncoordinated scheme, the social cost is uniquely determined for all cases with respect to the consumers behavior (e.g., risk-seeking and risk-conservative), risk-aversion degree values and energy consumption values $E_0$, $E_1$ except the following one. Specifically, for the risk-conservative consumers, the social cost depends on the choice of $p^{ES,NE}$ (Eq. \eqref{eq:social_cost_es_extra_demand}). The latter dependence is of interest under the conditions of the first line of  Table \ref{table_eq_comp_pro}, since it is the only case where there exist multiple combinations of probabilities that can lead to equilibria. We can obtain the worst social cost by  comparing the cases (i) maximum value of $p_{RES,0}^{ES,NE}$ and minimum of $p_{RES,1}^{ES,NE}$ (from the ranges in Eqs. \eqref{eq:prop_alloc_eq_bounds_0_extra_demand}, \eqref{eq:prop_alloc_eq_bounds_1_extra_demand}), (ii) minimum value of $p_{RES,0}^{ES,NE}$ and maximum of $p_{RES,1}^{ES,NE}$, choosing the one that leads to the highest social cost.
%
%%\emph{Price of Anarchy:} %Concerning the (in)efficiency of equilibria, 
%%By Section \ref{sec:eq_sharing_eq_extra_demand}, under risk-seeking consumers, the equilibrium states are possible if $E_0=E_1$ which returns $\textit{PoA}^{ES}=\textit{PoA}^{PA}$. On the other hand, under risk-conservative consumers,  %equilibrium states are possible also under asymmetric energy consumption profiles. In this case, 
%%the social cost is a non-increasing function of the competing probability of the competitors of high energy demand (\ie $\frac{d C(p^{ES,NE})}{d p^{ES,NE}_{RES,1}}\leq 0$) and therefore the worst-case equilibrium occurs at $p'$ with $p'_{RES,1}=min(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=max (p^{ES,NE}_{RES,0})$). By (\ref{eq:social_cost_es_extra_demand}), the associated PoA is 
%%
%%
%%\vspace{-5pt}
%%\small
%%\begin{eqnarray}
%% \hspace{-5pt} \textit{PoA}^{ES}  &=& \frac{C(p')}{C(p^{ES,OPT})}
%%\label{eq:poa_es}
%%\end{eqnarray}
%%\normalsize
%
%%where both the social costs $C(p')$ and $C(p^{ES,OPT})$ are derived by (\ref{eq:social_cost_es_extra_demand}).
%
%%\subsection{Decentralized Coordination Mechanisms}\label{sec:opt_decentral_no_extra_demand}
%
%%Although the centralized coordination mechanisms ensure optimal efficiency in the energy source allocation, they need to pursue incentives that would engage the autonomous and selfish consumers into socially efficient actions. Otherwise, supervisory implementations need to vouch for system stability and robustness, since selfish behaviors can undermine its performance significantly. The analysis in Section \ref{sec:uncoordinated_extra_demand} suggests that two important factors \emph{under the control} of micro-grid operator(s), affect the game equilibrium competing probabilities. These factors are the renewable energy capacity, $\mathcal{ER}$, and the applied pricing scheme on the two energy sources. Typically, in the long-term, the operator copes with the energy demand and the emerging inefficiencies through strategic planning of $\mathcal{ER}$, involving re-dimensioning of the distribution network side (\eg solar panels or wind turbines). Whereas, in the short-term, it can do so by manipulating the prices charged for the two types of energy sources. In the sequel, we systematically study conditions on $\mathcal{ER}$ and pricing that optimize the distributed energy source selection in large-scale settings where both the aggregate demands shaped by low-to-moderate and high energy consumers exceed $\mathcal{ER}$.
%%
%%\subsubsection{Proportional Allocation}\label{sec:opt_pa_decentral_no_extra_demand}
%%
%%%On the one hand, by Sections \ref{sec:prop_alloc_eq}, under proportional allocation the competing influences are balanced if $rse^{NE}_{\vartheta_i}(\cdot)=rse^{PA}_{\vartheta_i}(\cdot)$. On the other hand, by equation (\ref{eq:optimal}), optimal utilization of renewable energy along with elimination of congestion penalties are possible if the renewable energy demand matches the supply.
%%%
%%%Overall, under the case of risk-seeking consumers, by equations (\ref{eq:prop_alloc_energy}), (\ref{eq:conditionEQ}) and (\ref{eq:optimal}) (alternatively by (\ref{eq:demand_pa_ne_no_extra_demand})), the uncoordinated energy source selection converges to the optimal coordinated energy source allocation only if $E_0=E_1=E$ and the renewable energy capacity is dimensioned according to
%%%
%%%\vspace{-5pt}
%%%\small
%%%\begin{equation}
%%%\mathcal{ER}^{OPT}=\frac{E \cdot N}{\frac{(\gamma-1)N}{(\gamma-\beta)}-(N-1)}
%%%\label{eq:optimal_ER_proportional_no_extra_demand}
%%%\end{equation}
%%%\normalsize
%%%
%%%or the charging costs satisfy
%%%
%%%\vspace{-5pt}
%%%\small
%%%\begin{equation}
%%%\frac{(\gamma-1)}{(\gamma-\beta)}\vert ^{OPT}=\frac{N-1}{N}+\frac{E}{\mathcal{ER}}
%%%\label{eq:optimal_pricing_proportional_no_extra_demand}
%%%\end{equation}
%%%\normalsize
%%
%%%Under the case of risk-conservative consumers, by equations (\ref{eq:prop_alloc_energy}), (\ref{eq:conditionEQ_extra_demand}) and (\ref{eq:optimal}) (alternatively by (\ref{eq:demand_pa_ne_extra_demand})), the uncoordinated energy source selection converges to the optimal coordinated energy source allocation if the renewable energy capacity is dimensioned according to
%%
%%By Section \ref{sec:opt_pa_central_no_extra_demand}, if $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, optimal RES utilization along with elimination of congestion penalties are possible if the renewable energy demand matches the supply. Jointly by Table \ref{table_eq_comp_pro} and Section \ref{sec:opt_pa_central_no_extra_demand}, the optimization of the uncoordinated energy source selection requires dimensioning and pricing according to
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\mathcal{ER}^{OPT}=\frac{E_{\vartheta_i}N}{\frac{(\gamma-1)N}{(\gamma-\epsilon_{\vartheta_i}\beta) }-(N-1)} >0
%%\label{eq:optimal_ER_proportional_extra_demand}
%%\end{equation}
%%\normalsize
%%
%%%or the charging costs satisfy
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}\vert ^{OPT}=E_{\vartheta_i}\left[\frac{N-1}{N}+\frac{1}{\mathcal{ER}}\right] >1
%%\label{eq:optimal_pricing_proportional_extra_demand}
%%\end{equation}
%%\normalsize
%%
%%with $\epsilon_{\vartheta_i}>\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. Namely, the distributed energy source selection is optimized by allocating the RES only to consumers with the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$. Likewise, in the symmetric case where $\epsilon_{\vartheta_i}=\epsilon'<\gamma/\beta$, $\forall i\in \mathcal{N}$, by Table \ref{table_eq_comp_pro}, (\ref{eq:prop_alloc_opt_bounds_0}) and  (\ref{eq:prop_alloc_opt_bounds_1}), the values for $\mathcal{ER}$ and charging costs that optimize the efficiency of equilibria are also given by (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) with $\vartheta_i=0$, when $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$ and $E_1 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$ or $E_1 > max(\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}, \frac{E_0}{1-\frac{(N-1)}{N}\frac{(\gamma-\epsilon_0\beta)}{(\gamma-1)}})$. 
%%
%%Furthermore, in settings where $\exists i \in \mathcal{N} : \epsilon_{\vartheta_i}\geq\gamma/\beta$, by Table \ref{table_eq_comp_pro} and (\ref{eq:prop_alloc_opt_p_cond}), the optimal distributed energy selection is possible by prioritizing the use of RES facility by consumers that incur the highest cost for reneging from competition, $\epsilon_{\vartheta_i}\beta$, yet not blocking the other consumption profile from the distribution of the remaining RES capacity. In this case the optimal values for the renewable energy capacity and the charging costs are determined according to (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) with $\epsilon_{\vartheta_i}<\epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$. If $\epsilon_{\vartheta_i}\geq\gamma/\beta$, $\forall i\in \mathcal{N}$, the dominant strategy for all consumer to compete for the renewable energy source is also the optimal one.
%%
%%The optimization of the distributed energy source selection by adopting particular values for the RES capacity and the charging costs, requires that both the equilibrium states and the optimal operation prioritize the same class(ses) of consumers in accessing the RES facility: if $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$, $E_1 > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$ and $\epsilon_0<\epsilon_1<\gamma/\beta$ or if 
%%$E_{\vartheta_i} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}$, $\forall i\in \mathcal{N}$, the price of the lack of coordination in the equilibria cannot be avoided by the decentralized mechanism. Overall, the use of optimal values for the RES capacity and the charging costs yields $\textit{PoA}^{PA} =1$, with the exception of settings where there is a unique optimal competing probability vector while the equilibrium states vary over a proper probability interval (\ie  when $E_0 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$,  $E_1 \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_1\beta)}$, $\epsilon_0<\epsilon_1$). In this case, the worst-case equilibrium occurs at $p'$ with $p'_{RES,1}=min(p^{PA,NE}_{RES,1})$ ($p'_{RES,0}=max (p^{PA,NE}_{RES,0})$) and the associated PoA is given by (\ref{eq:poa_pa}).
%%
%%%while they do not break condition (\ref{eq:relation_E_0_E_1_pa_ne_extra_demand}) that dictates the relation between $E_0$ and $E_1$ factoring in the renewable energy capacity and the charging costs. 
%%
%%%Ultimately, these values for the renewable energy capacity and charging costs optimize the efficiency of equilibria, yielding $\textit{PoA}^{PA} =1$.
%%
%%
%%\subsubsection{Equal Sharing}\label{sec:opt_es_decentral_no_extra_demand}
%%
%%By Section \ref{sec:eq_sharing_eq_extra_demand}, in the distributed energy source selection by risk-seeking consumers the equilibrium states under equal sharing and proportional allocation coincide, and hence the RES capacity and the charging costs that optimize the efficiency of the uncoordinated selection process ($\textit{PoA}^{ES} =1$) are given by equations (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}).
%%%By Section \ref{sec:eq_sharing_eq_extra_demand}, 
%%When the consumers are risk-conservative, a trivial but expensive methodology to optimize the distributed energy source selection amounts to increasing $\mathcal{ER}$ to guarantee that the faire shares suffice to serve all requests, \ie $\mathcal{ER}/N \geq E_1$. Alternatively, in settings with $\epsilon_{\vartheta_i}<\gamma/\beta$, $\forall i\in \mathcal{N}$, by Tables \ref{table_eq_comp_pro} and \ref{tb:opt_es_extra}, the decentralized optimization of energy source selection is realized under the same conditions as in proportional allocation (Ref. Section \ref{sec:opt_pa_decentral_no_extra_demand}).
%%
%%Otherwise, in settings where $\exists \epsilon_{\vartheta_i}, \epsilon_{\vartheta_j}:\epsilon_{\vartheta_i}\geq\gamma/\beta> \epsilon_{\vartheta_j}$, $i,j \in \mathcal{N}$, by Tables \ref{table_eq_comp_pro} and \ref{tb:opt_es_extra},  
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\mathcal{ER}^{OPT}=\frac{N}{\frac{(\gamma-1)N}{(\gamma-\epsilon_{\vartheta_j}\beta) E_{\vartheta_j}}-\frac{(N-1)}{E_{\vartheta_i}}} > 0
%%\label{eq:optimal_ER_ES_extra_demand1}
%%\end{equation}
%%\normalsize
%%
%%\vspace{-5pt}
%%\small
%%\begin{equation}
%%\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}\vert ^{OPT}=E_{\vartheta_j}\left[\frac{N-1}{NE_{\vartheta_i}}+\frac{1}{\mathcal{ER}}\right] > 1 
%%\label{eq:optimal_pricing_ES_extra_demand1}
%%\end{equation}
%%\normalsize
%%
%%which return $\textit{PoA}^{ES} =1$. In addition, by Table \ref{table_eq_comp_pro} and Section \ref{sec:opt_es_central_no_extra_demand}, if $\epsilon_{\vartheta_i}\geq\gamma/\beta$, $\forall i\in \mathcal{N}$, the dominant competing strategy equals to the optimal one.
%%
%%In a last note, the benefit of these decentralized coordination approaches can be also quantified by the Price of Stability (\textit{PoS}) which is a measure of inefficiency designed to differentiate between games in which \textit{all} equilibria are inefficient and those in which \textit{some} equilibria are inefficient \cite{Nisan07}. It is a ratio between the best objective function value at equilibrium and that of the optimal outcome. In the energy source selection game, with parametrization according to (\ref{eq:optimal_ER_proportional_extra_demand}) and (\ref{eq:optimal_pricing_proportional_extra_demand}) or (\ref{eq:optimal_ER_ES_extra_demand1}) and (\ref{eq:optimal_pricing_ES_extra_demand1}), the best-case equilibrium emerges at the optimal competing probabilities. Therefore, these decentralized coordination approaches guarantee $\textit{PoS}=1$.
%%
%% %emerges at $p'$ with $p'_{RES,1}=supremum(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=infimum (p^{ES,NE}_{RES,0})$) or $p'_{RES,1}=infimum(p^{ES,NE}_{RES,1})$ ($p'_{RES,0}=supremum (p^{ES,NE}_{RES,0})$), respectively. Therefore, these decentralized coordination approaches guarantee $\textit{PoS}=1$.
%%
%%


==> coordinated_lesia.tex <==
\section{Centralized Energy Source Allocation}\label{sec:coordinated}

In this section, we study the centralized mechanism that allocates the different energy sources to the $N$ consumers of the micro-grid.

\subsection{Optimization Problem Formulation}


In practice, in the centralized mechanism, all consumers, $i \in \mathcal{N}$ with type $\vartheta_i \in \Theta$ issue energy demand requests $E_{\vartheta_i}$ to a central micro-grid operator that optimally processes their requests and allocates resources. Therefore, the aggregate amount of day-zone loads is equal to $D^{Total}$. In line with the decentralized mechanism, each consumer type $\vartheta_i \in \Theta$ is associated with a risk aversion coefficient $\epsilon_{\vartheta_i} \geq 1$. If its consumption is allocated in the day-zone, it is equal to $\epsilon_{\vartheta_i}E_{\vartheta_i}$, while if it is allocated in the night-zone, it is equal to $\epsilon_{\vartheta_i}E_{\vartheta_i}$. The central mechanism then optimally dispatches the loads between the day-zone and the night-zone, in order to minimize the total minimizing the social cost  $C^{OPT}(\mathbf{p}^{OPT})$ for all the consumers.
%As the centralized mechanism aims at minimizing the social cost of all consumers, if the aggregate amount of day-zone loads does not exceed $\mathcal{ER}$, they are all allocated RES production during the day-zone. Otherwise, certain consumers are allocated the RES production during the day-zone and others are shifted to the night-zone so as to minimize the social cost. %This means that the centralized coordinator allocates a total RES production in the day-zone equal to $D^{OPT}= \min \left\{D^{Total},\mathcal{ER} \right\}$, in all considered cases and under all allocation policies.
The decision variables of this optimization problem are the optimal probability distributions ($p^{OPT}_{RES,\vartheta_i}$, $p^{OPT}_{nonRES,\vartheta_i}$) for all consumers $i \in \mathcal{N}$, where $p^{OPT}_{RES,\vartheta_i}$ ($p^{OPT}_{nonRES,\vartheta_i}$) is the optimal probability that consumer $i$ with type $\vartheta_i$ engages its load during day-zone (night-zone). And, the vector $\mathbf{p^{OPT}}$ is defined similarly to $\mathbf{p^{NE}}$.

%\subsection{Problem description}

%In the micro-grid with $N>1$ (eligible) consumers which have access to multiple sources of energy described in Section \ref{sec:game}, 
%The allocation of the available RES, $\mathcal{ER}$, to the $N$ consumers could be carried out optimally through a fully coordinated centralized approach. 
%Typically, smart grid-enabled information flow from and to the consumers could be exploited to ensure that (a) the RES is fully used and fairly allocated among the consumers, and (b) the social cost of the micro-grid is minimized.

The social cost is defined as
\begin{small}
\begin{align}
C^{OPT}(\mathbf{p}^{OPT}) &=   \min\Bigl\{ N \sum_{{\vartheta_\ell} \in \Theta} r_{\vartheta_\ell} p_{RES,{\vartheta_\ell}}^{OPT}  E_{\vartheta_\ell}, \mathcal{ER}\Bigr\}  c_{RES} \nonumber \\ & \max \Bigl\{ N \sum_{{\vartheta_\ell} \in \Theta} r_{\vartheta_\ell} p_{RES,{\vartheta_\ell}}^{OPT}  E_{\vartheta_\ell}- \mathcal{ER},0\Bigr\}  c_{nonRES}\nonumber \\
& + N  \sum_{{\vartheta_\ell} \in \Theta} r_{{\vartheta_\ell} }p^{OPT}_{nonRES,{\vartheta_\ell}}\varepsilon_{{\vartheta_\ell} }E_{{\vartheta_\ell}} c_{nonRES,N},
 \label{eq:social_cost_x_opt}
 \end{align}
\end{small}
%where $N  \sum_{{\vartheta_\ell}\in \Theta} r_{\vartheta_\ell} p_{RES,{\vartheta_\ell}}^{OPT}  E_{\vartheta_\ell} $ represents the total RES production allocated in the day-zone, and $N  \sum_{{\vartheta_\ell} \in \Theta} r_{{\vartheta_\ell} }p^{OPT}_{nonRES,{\vartheta_\ell}}\varepsilon_{{\vartheta_\ell} }E_{{\vartheta_\ell}}$ represents the total nonRES production allocated in the night-zone. %The first summand refers to the consumers who are served by low-cost RES capacity during the day-zone. The second summand is for the consumers who are served $nonRES$ duing the night-zone. 
%In other words, the part of the optimal social cost that corresponds to the day-zone peak-load production will be zero. %The social costs under the PA and ES policies are defined similarly to Eqs. \eqref{eq:social_cost_pa_extra_demand} and \eqref{eq:social_cost_es}, respectively. 

The optimal solution of centralized mechanism will provide a benchmark against which to evaluate the side-effects that stem from the distributed, uncoordinated energy source selection, in terms of social cost. The (in)efficiency of equilibrium strategies in the decentralized, uncoordinated mechanism is quantified by the Price of Anarchy (PoA) \cite{Koutsoupias09}. The PoA is expressed as the ratio of the worst case social cost among all NE over the optimal-minimum social cost of the centralized mechanism. In order to compute the PoA for each examined case, we should compute the mixed strategy equilibrium that leads to the worst social cost, denoted as $C^{NE}_w$, for this case. PoA is computed as follows: %with respect to the consumers behavior (e.g., risk-seeking and risk-conservative), risk-aversion degree values and energy consumption values $E_0$, $E_1$.

%\vspace{-5pt}
\small
\begin{align}
 \hspace{-5pt} \textit{PoA}  = \frac{C^{NE}_w}{C^{OPT}(\mathbf{p^{OPT}})},
\label{eq:poa_pa}
\end{align}
\normalsize

To obtain $C^{NE}_w$ when there exist multiple possible NEs (e.g., in cases 2 and 4), we can solve a simple optimization problem to minimize the social cost $C^{NE}(\mathbf{p^{NE}})$ with respect to $\mathbf{p^{NE}}$ and subject to the corresponding probability constraints using a software optimization tool. Importantly, minimizing $C^{NE}(\mathbf{p^{NE}})$  is equivalent to minimizing the night-zone cost. The last observation is due to the fact that the demand $D^{NE}$ is constant with respect to $\mathbf{p^{NE}}$. Also, in the special case of the risk-seeking consumers, from Eq. \eqref{eq:social_cost_pa_sc}, the social cost is constant with respect to the probabilities $\mathbf{p^{NE}}$ for each case of energy profile values. Thus, $C^{NE}_w$ is given by Eq. \eqref{eq:social_cost_pa_sc}.




==> game.tex <==
\section{Modeling the energy source selection}\label{sec:game}
%\textbf{we need to specify a time-unit of taking the decisions: if we take them only once then (i) ER cannot be known, (ii) why not centralized approach. This is studied for one time interval. Can I decide at a next time interval to move back some loads sent to night rate at a previous interval to ER - intra-day re- scheduling per interval? Nice to describe how this is done. }

We consider a smart-grid with $N$ (eligible) consumers. Let $\mathcal{ER}$ stand for the available RES capacity in energy units (\eg kWh) for the considered time-period in the day-zone. Also, we define the following per unit of energy cost values, namely, (i) $c_{RES}$ for RES, (ii) $c_{nonRES,N} = \beta \cdot c_{RES}$, for night-zone nonRES with $\beta>1$, and (iii) $c_{nonRES,D}= \gamma \cdot  c_{RES}$ for day-zone nonRES with $ \gamma>\beta$. Notice that an \emph{excess penalty cost}, equal to $(\gamma-\beta) \cdot c_{RES}$ per unit of energy load, will be paid by consumers that was engaged in the day-zone but not served due to the limited RES capacity. % and captures the impact of congestion (in case of the uncoordinated competition) for RES. 
All aforementioned costs, as well as the amount of the available RES, $\mathcal{ER}$, are assumed as known to the consumers. %We also assume that the consumers do not increase their demand when opting for the night-zone. 
%The challenge addressed in this paper is finding a distributed and uncoordinated scheduling of the consumer loads in day and night-zones so that the consumers' average cost is minimized. Based on the prices, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. %More specifically, we solve the problem of the energy source selection, between RES and night-zone nonRES, by the consumers themselves. %We first present a short discussion on a benchmark centralized solution and afterwards we will discuss the simpler to implement distributed one. 
%
%In time zones when the capacity of RES suffices to serve the entire energy demand, consumers can readily opt for using it and gain the price differential between the two resources. When, however, the demand exceeds the limited RES, an inherent competition emerges that should be factored by consumers in their decision to opt for requesting this resource or not at the particular time period. The underlying assumption is that the decision to opt for the finite RES bears the risk of experiencing the congestion penalties induced by the lack of coordination and pay for the more expensive, top-priced nonRES. Essentially, the main dilemma faced by consumers is whether to compete or not for requesting RES or settle for less favoured time zones and pay for medium-priced energy (assumed being covered by a nonRES facility).
%
%In order to analytically investigate the suffered congestion penalties due to the uncoordinated access to the limited resource, it is important to identify and model those key features and critical parameters that tune the intensity of competition. In this respect, we may consider $N$ consumers that decide between RES and nonRES. The first facility is capacity-constrained and able to serve a total energy demand of $\mathcal{ER}$ energy units (\eg kilowatt-hours, kWh) while the second one responds to every possible level of energy demand, yet heavily burdens the environment producing large amounts of pollutants. In the pricing arena, RES is offered at $c_{RES}$ cost units, whereas for nonRES different rates are used for daily and night energy consumption: moderate-priced night energy rate of $c_{nonRES,N} = \beta \cdot c_{RES}, \beta>1$, units and top-priced daily energy rate of $c_{nonRES,D}= \gamma \cdot  c_{RES}, \gamma>\beta$, units. The excess penalty cost $\delta\cdot c_{RES}$, with $\delta=\gamma-\beta>0$, captures the impact of congestion for RES.

%\textbf{Optimal coordinated RES allocation:} 
The allocation of the available RES, $\mathcal{ER}$, to the consumers could be carried out optimally through a fully coordinated centralized approach. %Typically, smart grid-enabled information flow from and to the consumers could be exploited to ensure that (a) the RES is fully used and fairly distributed among the consumers and (b) no consumer would pay the excess congestion penalty. 
This can be implemented by having consumers issue energy demand requests to a central server that processes the requests; if the aggregate amount of loads does not exceed $\mathcal{ER}$, they are all selected during the day-zone, otherwise, certain loads are selected so that their aggregate amount is less or equal to $\mathcal{ER}$ and the remaining non-selected loads are shifted to the night-zone. Besides the increased communication and processing requirements, a coordinated RES allocation is a complex process that needs to take into account fairness criteria, the complex interplay between energy consuming devices, %the heterogeneity of the micro-grid environments often consisting of fairly diverse components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements, weather conditions, 
user preferences/comfort, \etc, and it is not scalable. In addition, a major concern of a centralized solution is the privacy of consumers, since they should reveal their demands/constraints to a central server. Also, there is no guarantee that consumers will report their demands truthfully.
%Note that when consumers increase their demand when avoiding the competition, the optimal allocation becomes more complex since it should compare the aggregate cost for consuming nonRES at day-zone against the aggregate cost for consuming (more) nonRES at night-zone. These decisions are communicated to the consumers through the smart-grid facility. 

%
%
%Under the optimal coordinated energy source allocation scheme, %the full information processing and decision-making tasks lie with a central entity.
%micro-grid operators %, operators of energy efficient neighbourhoods and operators of building blocks that host smart metering 
%use the smart grid-related information so as to coordinate the actions of all different stakeholders involved and secure that (a) the local RES - and storage systems - are optimally used and fairly distributed among consumers and (b) no one would pay the excess congestion penalty. In essence, individual customers/consumers that range from owners/operators of large building and facilities to house customers, are expected to issue energy demand requests to a central server, which monitors RES, possesses precise information about its availability, and assigns it so that the aggregate consumers' cost is minimized. Ideally, the efficient exploitation of the smart meter attributes requires the use of a highly intelligent mechanism which takes into account the complex interplay between energy consuming devices, weather conditions, building dynamics, user preferences and comfort, grid status, availability of RES or storage systems \etc.
%
%Overall, in an micro-grid environment where the aggregate demand exceeds the RES capacity of $\mathcal{ER}$ energy units, %with RES capacity of $\mathcal{ER}$ energy units, whereby such an coordination system serves the energy requests of $N$ consumers that jointly shape an energy demand exceeding the RES capacity, 
%exactly $\mathcal{ER}$ units of demand would be directed to RES and no one would pay the excess congestion penalty cost. Advanced decentralized realizations of optimal coordination mechanisms may optimally shape the $\mathcal{ER}$ capacity, pricing and the energy demand of all different consumers within the operator's entity so as the locally available RES is exploited to the maximum while the needs from purchasing from the top-priced conventional grid are minimized.

%\textbf{Uncoordinated energy source selection:} As already mentioned, the design and implementation of a coordinated energy source selection is complex due to the required information exchange, fairness criteria to be considered, heterogeneity of the micro-grid environments (often consisting of fairly diveRES components such as electric cars, wind turbines, solar farms and all kinds of different appliances with various capabilities and requirements), \etc. 
Consequently, in this paper we investigate a simpler to implement distributed, uncoordinated energy source selection approach. Each consumer acts selfishly aiming at minimizing the cost of the acquired energy. Based on the prices' definitions, if the consumers' average cost is minimized, the amount of RES actually used (and not curtailed) should be maximized. As aforementioned in the introduction, the intuitive tendency to opt for RES combined with its scarcity foster the tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task. Thus, the decision-making on energy source selection can be formulated in game-theoretic terms, whereby $N$ rational players/consumers compete against each other for a capacity of $\mathcal{ER}$ low-cost energy units. We will compare the optimal (theoretical) performance (expressed in terms of the minimum average aggregate consumer cost) achieved via the centralized coordinated energy allocation, against the one under the distributed, uncoordinated approach proposed in this paper. 



%Advanced decentralized realizations of the aforementioned optimal centralized coordination may also be considered, but this is outside the focus of this paper. We are only interested in comparing the optimal (theoretical) performance (expressed in terms of the minimum average aggregate consumer cost) delivered through centralized or decentralized coordinated energy allocation, against that under the (simpler to implement) uncoordinated approach considered in this paper. 

%
%Typically, the research in the optimization of energy grid system operation, amounts to defining and solving a system-level optimization problem based on a centralized objective function. However, under heterogeneous micro-grid networks, often consisting of different components such as electric cars, diesel generators, wind turbines, solar farms and all different appliances with various capabilities and objectives, specific objective function for each individual component should be taken into account. Indeed, considering the demand side, in the absence of central coordination, each consumer acts selfishly aiming at minimizing the cost of the acquired energy. The intuitive tendency to opt for RES combined with its scarcity, foster tragedy of commons effects and highlight the game-theoretic dynamics behind the energy source selection task.
%
 %coming up with optimal decisions for operating their associated energy consuming devices. 
%In doing so, they are assumed here to hold precise information about the RES capacity and the pricing on all energy sources involved (RES, day and nigh time grid energy). They also may or may not hold precise information about the actual demand, \ie competition. These assumptions are fairly realistic and feasible since the decision-making task can be assigned to intelligent meters that leverage the available information (through the communication network layer within the smart grid infrastructure) to perform complex computations and best respond to others' actions. Furthermore, these meters may account for user preferences and comfort in the reasoning process. To this end, we assume \textit{two} generic energy consumption profiles corresponding to low-to-moderate and high consumption level energy users.

\vspace{-2pt}
\subsection{Game setting}\label{sec:game_definition}

Overall, the distributed, uncoordinated decision-making on energy source selection can be expressed via the following game: 
\begin{definition}\label{def:energy_source_game}
An \emph{Energy Source Selection Game} is a tuple
\\$\Gamma=(\mathcal{N}, \mathcal{ER}, \{\vartheta_{i}\}_{i\in \mathcal{N}}, \{A_{i}\}_{i\in\mathcal{N}},  \{w_{A_{i},\vartheta_{i}}\}_{i\in \mathcal{N}})$, where:
\begin{itemize}
\item $\mathcal{N}=\{1,...,N\}$, $N>1$, the set of energy consumers/users acting as players,
\item $\mathcal{ER}>0$, the RES capacity in energy units,
\item $\vartheta_{i} \in \Theta=\{0,1,...,M-1\}$ is the type of user $i$ ($i\in \mathcal{N}$) corresponding to an energy consumption profile (load) with demand of $E_{\vartheta_i}$ energy units. It should hold that $M \leq N$ and it is assumed that $E_0<E_1<...<E_{M-1}$, %where $0$ ($1$) stands for low-to-moderate (high) energy level users with demand of $E_0$ ($E_1$, $E_1 \geq E_0$) energy units,
\item $A_{i} $ is the pure strategy of player $i$ taking values in the set of potential pure strategies $\mathcal{A}=\{RES,nonRES\}$ (same for all consumers $i\in \mathcal{N}$), consisting of the choices ``low-priced renewable-source energy'' (RES) and ``medium-priced night-zone non-renewable-source energy'' (nonRES),
%\item $s_{i}: \Theta \rightarrow A$, the strategy function for each consumer $i\in \mathcal{N}$,
\item $w_{RES,\vartheta_i}$, $w_{nonRES,\vartheta_i}: \mathbb{R}^2 \rightarrow \mathbb{R}$ are cost functions indexed by the pure strategy RES or nonRES, and the user type $i\in \mathcal{N}$. 
\end{itemize}
\end{definition}
In addition, 
\begin{itemize}
\item a consumer has an energy demand level $E_{\ell}$ with probability $r_{\ell}$, where $\sum_{\ell\in \Theta} r_{\ell}=1$,
\item $\mathbf{p}_{\boldsymbol \vartheta_i}=(p_{RES,\vartheta_i}, p_{nonRES,\vartheta_i})^T$ is the mixed strategy of user $i$ with profile $\theta_i$ and let $\mathbf{p}=(\mathbf{p_0}^T;\mathbf{p_1}^T;...;\mathbf{p_{M-1}}^T)$,
\item $\upsilon_{RES, \theta_i}(p)$,  $\upsilon_{nonRES, \theta_i}(p)$ are expected cost values for each pure strategy RES, nonRES, respectively, of user $i$ with type $\theta_i$ given the mixed strategies of all other users; the expected value is over both the strategy choice by other consumers and their energy profile.   
%\item $c_{i}^{N_0}(A_i,\vartheta_i)$ are cost functions under particular type, $\vartheta_i$, and strategy, $A_i$, that are basically determined based on $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$.
%$c_{i}^{(\cdot)}(s(\vartheta),\vartheta)= c_{i}^{(\cdot)}(s_{i}(\vartheta_{i}),s_{-i}(\vartheta_{-i}),\vartheta_{i},\vartheta_{-i})$, are the expected cost functions for each consumer $i\in \mathcal{N}$, for every type profile $\vartheta\in \times_{k=1}^{N}\Theta_{k}$ and strategy profile $s(\vartheta)\in \times_{k=1}^{N}S_{k}$, ($c_{i}^{N_0}(s(\vartheta),\vartheta)$ are cost functions under particular type, $\vartheta$, and strategy, $s(\vartheta)$, profile with $N_0=N-\sum_k \vartheta_k$), that are functions of $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$,
\end{itemize}

The number of users with energy profile $E_\ell$, $\ell \in \Theta$, taking action $RES$, excluding player $i$, is denoted as $n_{\ell}$. %and it is equal to $\sum_{j \in \mathcal{N}\setminus {i}} \mathbf{1}_{(A_j=RES)}\cdot \mathbf{1}_{(\theta_j=\ell)}$. %and similarly the corresponding number of competitors of high energy profile is $n_{1}$ ($=\sum_{j \in \mathcal{N}\setminus {i}} A_j \mathbf{1}_{(\theta_j=1)}$). 
The cost function $w_{RES,\vartheta_i}(.)$, is non-decreasing with the {number} of players competing for RES ($n_{\ell}$,  $\ell \in \Theta$) and has the same value for all players of the {same} energy profile that play the same strategy. Let us denote as $\mathbf{n}=(n_0, n_1,..., n_{M-1})^T$. %consumers who decide to compete for RES undergo the risk of incurring congestion penalties. 
In addition, $w_{RES,\vartheta_i}(.)$ is determined %based on the actions taken by the entire population, on the one side, and 
based on the allocation rule that the micro-grid operator adopts to distribute RES among those who compete for it. %, on the other side. %We denote an action profile by the vector $a=(a_{i},a_{-i})\in\times_{k=1}^{N}A_{k}$, where $a_{-i}$ denotes the actions of all other consumers but player $i$ in the profile $a$. The full set of $2^N$ different action profiles maps into $(N_0+1)(N-N_0+1)$ different action \emph{meta-profiles}, where $N_0$ is the number of low-to-moderate energy consumption users. Each meta-profile $a(k_0,k_1)$, with $k_0$, $k_1$ denoting the number of competitors of low-to-moderate and high energy profile, respectively, encompasses all different action profiles that correspond to the same number of consumers of the two energy profiles competing for RES. The expected costs for these $k_0$, $k_1$ consumers and for the $N-(k_0+k_1)$ ones choosing directly the medium-priced nonRES alternative are functions of $a(k_0,k_1)$ rather than the exact action profile.
Thus, the cost for a consumer $i\in \mathcal{N}$ of consumption profile $\vartheta_i$ (and associated energy demand $E_{\vartheta_i}$) that plays the action $RES$ is:
\begin{small}
\begin{align}
w_{RES,\vartheta_i}(n) =
rse_{\vartheta_i}(n) \cdot c_{RES} + (E_{\vartheta_i}-rse_{\vartheta_i}(n) ) \cdot c_{nonRES,D},
\label{eq:RES_cost}
\end{align}
\end{small}
where $rse_{\vartheta_i}(n) $ is the amount of RES allocated to consumer profile $\vartheta_i$. Note that all consumers $j \neq i, ~j \in \mathcal{N}$ with $\vartheta_j=\vartheta_i$ and strategy RES are granted with the same amount of RES. On the other hand, the cost for those avoiding competition, $w_{nonRES,\vartheta_i}$, is oblivious to others' actions, that is, 
%\vspace{-7pt}
%\small
\begin{equation}
w_{nonRES,\vartheta_i}=E_{\vartheta_i} \cdot c_{nonRES,N}.
\label{eq:nonRES_cost}
\end{equation}
\normalsize
%In general, the cost $c_i^{N_0}(a_i,a_{-i})$ for consumer $i$ under the action profile $a=(a_i,a_{-i})$ is
%
%%\vspace{-10pt}
%\small
%\begin{eqnarray}
%\hspace{-1pt}c_{i}^{N_0}(a_{i},a_{-i})=\left\{
%\begin{array}{l l}
%\hspace{-5pt}w_{RES,\vartheta_i}(N_{RES,0}(a), n_{1}(a)), \text{if~ $a_{i}=RES$} \nonumber\\
%\hspace{-5pt}w_{nonRES,\vartheta_i}, \text{if~ $a_{i}=nonRES$} \nonumber\\
%\end{array} \right.
%\label{equ:consumer_cost_profile}
%\end{eqnarray}
%\normalsize
%
%where $N_{RES,0}(a), n_{1}(a)$ are the numbers of competitors of low-to-moderate and high energy profile \textit{but} player $i$, respectively, under action profile $a$.
Besides the two pure strategies, RES, nonRES, the consumers may also randomize over them\footnote{Note that a pure strategy is a special case of a mixed strategy.}. We mainly draw our attention on symmetric mixed strategies for each energy consumption profile, since these can be more helpful in dictating practical strategies in real systems. In particular, as defined above a player's \emph{mixed strategy} corresponds to a probability distribution $\mathbf{p}_{\boldsymbol \vartheta_i}$. %=(p_{RES,\vartheta_i},p_{nonRES,\vartheta_i})$, where $p_{RES,\vartheta_i}$ and $p_{nonRES,\vartheta_i}$ are the probabilities of selecting the pure strategies RES and nonRES, respectively, with $p_{RES,\vartheta_i}+p_{nonRES,\vartheta_i}=1$ ($\theta_i \in \Theta$). %Also, let $p=(p_0^T;p_1^T)$ be the matrix with lines the symmetric mixed strategies for each energy profile, namely, $p_0=(p_{RES,0}; p_{nonRES,0})$ and $p_1=(p_{RES,1}; p_{nonRES,1})$. %associated with the two energy profiles. 
Assume that consumers play the mixed-action strategy $\mathbf{p}$. In this case, the expected costs for player $i$, with energy profile $\theta_i$, when playing RES (nonRES) is %is a weighted sum of the cost functions $w_{RES,\vartheta_i}(\cdot)$ and $w_{nonRES,\vartheta_i}(\cdot)$ and is given by
%\vspace{-15pt}
%\small
%\begin{eqnarray}\label{eq:costs_symRES}
%    c_{i}(RES,p, p_{0}, p_{1}) = \sum_{N_0=0}^{N-1}\sum_{N_{RES,0}=0}^{N_0}\sum_{n_{1}=0}^{N-1-N_0}    w_{RES,\vartheta_i}(\cdot)  && \nonumber\\
%    \cdot B(n_{1};N-1-N_0,p_{RES,1}) \cdot  B(N_{RES,0};N_0,p_{RES,0}) && \nonumber\\
%      \cdot B(N_0;N-1,p) &&
%    \vspace{-10pt}
%\end{eqnarray}
%\normalsize
%\begin{align}
%   \upsilon_{ \theta_i}^{N_0}(p_0,p_1) = &  p_{RES,\theta_i} ~\upsilon_{RES, \theta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\theta_i} \upsilon_{nonRES, \theta_i}^{N_0}(p_0,p_1),\label{eq:costs_tot}
%\end{align}
%\noindent where the expected costs of the pure strategies RESs, nonRES of consumer $i$ are expressed as
\begin{align}& \upsilon_{RES, \theta_i}(\mathbf{p})=  \sum_{N_{0}=0}^{N}~ \sum_{N_{1}=0}^{N-N_0} ... \sum_{N_{M-1}=0}^{N-\sum_{k=0}^{M-2}{N_k}}\nonumber\\  & \Bigl( \sum_{n_{0}=0}^{N_0-\mathbf{1}_{(\theta_i=0)}}~\sum_{n_{1}=0}^{N_1-\mathbf{1}_{(\theta_i=1)}}...  \sum_{n_{M-1}=0}^{N_{M-1}-\mathbf{1}_{(\theta_i=M-1)}} ~w_{RES,\vartheta_i}(n) \cdot \nonumber\\
 &B(n_{0};N_0-\mathbf{1}_{(\theta_i=0)},p_{RES,0}) \cdot \nonumber \\& B(n_{1};N_1-\mathbf{1}_{(\theta_i=1)},p_{RES,1}) \cdot... \nonumber \\& B(n_{M-1};N_{M-1}-\mathbf{1}_{(\theta_i=M-1)},p_{RES,M-1})\Bigr) \cdot... \nonumber \\&B(N_0;N,r_0)B(N_1;N,r_1)...B(N_{M-1};N,r_{M-1}),  \label{eq:costs_symRES}
\end{align}
\begin{align}
\label{eq:costs_symnonRES}
   \upsilon_{nonRES, \theta_i}(\mathbf{p}) = w_{nonRES,\vartheta_i},
\end{align}
\noindent where $N_{\vartheta_i}$ is the number of consumers of type $\theta_i\in \Theta$, $B(n_{0};N_0-\mathbf{1}_{(\theta_i=0)},p_{RES,0}) $ is the value of the Binomial probability distribution with parameters $N_0-\mathbf{1}_{(\theta_i=0)}$ and $p_{RES,0}$, for $n_{0}$ consumers of energy profile $E_0$ competing for RES, and $B(N_0;N,r_0)$ is the value of the Binomial distribution for $N_0$ consumers of energy profile $E_0$ with parameters $N$ and $r_0$. %and $B(N_0;N-1,p)$ is the Binomial probability distribution with parameters $N-1$ and $p$, for $N_0$ consumers of low-to-moderate energy consumption users.

The Energy Source Selection Game has at least one (mixed) Nash Equilibrium, as it is a game with finite set of players and finite strategy sets (Nash's original result). To derive the equilibria, we recall that any mixed strategy equilibrium $\mathbf{p^{NE}}=(\mathbf{p_0^{NE}}, \mathbf{p_1^{NE}}, ..., \mathbf{p_{M-1}^{NE}})^T$ must fulfill

\vspace{-5pt}
\small
\begin{equation}\label{eq:cost_equality_mixed}
\upsilon_{RES, \theta_i}(\mathbf{p^{NE}})= \upsilon_{nonRES, \theta_i}(\mathbf{p^{NE}}), ~\forall \theta_i \in \Theta.
\end{equation}
\normalsize

Namely, the expected costs of each pure strategy that belongs to the support of the equilibrium mixed strategy are equal. %By Eq. (\ref{eq:costs_symnonRES}), the expected cost of action nonRES, $ \upsilon_{nonRES, \theta_i}(p_0^{NE}, p_1^{NE})$, is insensitive to $N_0$ (or $N-N_0$), that is, the cardinality of the two sets of consumers. 
%In addition, in order to accommodate different risk attitudes, it becomes $c_{i}^{(\cdot)}(nonRES,p) = (\epsilon_{\vartheta_i}  E_{\vartheta_i})  c_{nonRES,N}$. 
%Likewise, by Definition \ref{def:energy_source_game}, the expected cost of action RES is given by $c_{i}^{(\cdot)}(RES,p) =\sum_{N_0=0}^{N}c_{i}^{N_0}(RES,p) B(N_0;N,r)$, where the cost $c_{i}^{N_0}(RES,p)$ follows equation (\ref{eq:costs_symRES}). 
The cost for the RES pure strategy, $\upsilon_{RES, \theta_i}(p^{NE})$, given by Eq. (\ref{eq:costs_symRES}), under large populations of consumers, can be approximated by

\vspace{-5pt}
\small
\begin{align}
&\upsilon_{RES, \theta_i}(\mathbf{p^{NE}})=w_{RES,\vartheta_i}(\mathbf{n}),\nonumber \\&
\mathbf{n}=(r_0 p_{RES,0}^{NE}, r_1 p_{RES,1}^{NE}, ...,  r_{M-1} p_{RES,M-1}^{NE})^T\cdot (N-1).\label{eq:gen_costs_symRES}
\end{align} \normalsize
%In the rest of the paper, we will apply the definition of $n$ of Eq. \eqref{eq:gen_costs_symRES}.


%As a result, the player $i$, with energy profile $\theta_i$, and mixed strategy $p_{\vartheta_i}=(p_{RES,\vartheta_i};p_{nonRES,\vartheta_i})$ will have an expected cost equal to
%\begin{align}
%   \upsilon_{ \theta_i}^{N_0}(p_0,p_1) = &  p_{RES,\theta_i} ~\upsilon_{RES, \theta_i}^{N_0}(p_0,p_1)  \nonumber \\&  + p_{nonRES,\theta_i} \upsilon_{nonRES, \theta_i}^{N_0}(p_0,p_1).\label{eq:costs_tot}
%\end{align}
\subsection{Risk Attitude of the Consumers}
%Various expressions of consumers' risk attitude are considered yielding different variants of the game prescribed under Definition \ref{def:energy_source_game}. 
In the game of Definition \ref{def:energy_source_game}, we take into account various risk attitudes of the consumers.  %Specifically, the risk attitude of a consumer is expressed by adjusting the reported energy demand to its level of risk. 
A \textit{risk-seeking} consumer when playing the RES strategy will gamble its total energy demand in the game; that is, it will attempt to have its entire possible energy demand served by the RES and minimize its cost. On the contrary, a \textit{risk-conservative} consumer with RES strategy gambles part of its possible total energy demand. 

The above described risk attitude is captured by adjusting the energy demand of consumer $i\in \mathcal{N}$ when served at the night zone as $\epsilon_{\vartheta_i} E_{\vartheta_i}$, where the parameter $\epsilon_{\vartheta_i}$ is the ``{risk-aversion degree}'' and $\epsilon_{\vartheta_i}\geq 1$. For example, $\epsilon_{\vartheta_i}=1$ in case of a risk-seeking consumer $i$ and $\epsilon_{\vartheta_i}>1$ in case of a risk-conservative consumer $i$. The consumer's $i$ energy demand when competing for RES remains equal to $E_{\vartheta_i}$. Note that we assume that consumers with the same energy profile $\theta_i$ will have the same risk attitude. In order to capture these risk attitudes, Eq. \eqref{eq:nonRES_cost} should take the form
\begin{small}
\begin{equation}
w_{nonRES,\vartheta_i}=\epsilon_{\vartheta_i} \cdot E_{\vartheta_i} \cdot c_{nonRES,N}.
\label{eq:nonRES_cost2}
\end{equation}
\end{small}

==> policies.tex <==
\subsection{Renewable Energy Allocation Policies}\label{sec:policies}

The allocation of scarce resources to human-driven agents with distinct demands, is challenging. In this paper, we examine two types of allocations with different fairness properties, namely, the proportional allocation and the equal sharing.%The engagement of humans (behind the machines) transfuse social features and require careful consideration of the fairness properties of the resource allocation policy, as it impacts on users' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

%In multiplexing settings, the division of scarce resources motivates a number of challenges with respect to the properties that should characterize the allocation mechanism. Most commonly, the allocation mechanisms pursue an utilitarian view of the allocation (\ie aggregation of agents' utility on the allocated resources). However, practical circumstances that engage humans (and machines) transfuse social features to the allocation process and raise some concerns about the level of fairness that should vouch for. The fairness properties of an allocation mechanism have a direct impact on agents' satisfaction, participation, compliance pervasion, and ultimately, on system's efficiency \cite{Busqu12}.

\paragraph{Proportional Allocation}\label{sec:prop_alloc}

The proportional allocation allocates resources in proportion to the consumer demand. Under this policy, the amount of RES received by a consumer of type $\vartheta_i$ is given by,
% all users a level of service proportional to their actual needs. In turn, applying this allocation rule in the distribution of RES capacity, consumers that compete for RES capacity are endowed with an amount of energy that is given by 

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
rse^{PA}_{\vartheta_i}(\mathbf{n}) &=& \frac{E_{\vartheta_i}}{\max(\mathcal{ER} ,(\sum_{\ell \in \Theta } n_{\ell  } E_{\ell  }+ E_{\vartheta_i })}\mathcal{ER},
\label{eq:prop_alloc_energy}
\end{eqnarray}
\normalsize

%where $n_0=n_{RES,0}$, $n_1=n_{RES,1}$ and 
where $\sum_{\ell \in \Theta } n_{\ell  } E_{\ell  }+ E_{\vartheta_i}$ is the total energy demand.

\paragraph{Equal Sharing}\label{sec:eq_sharing}

Under equal sharing, all competing consumers will obtain the same amount of resources (as long as they have a need for). Under this policy, the amount of RES received by a consumer of type $ \vartheta_i$ is given by,
%benefits from accessing a particular service. In the energy front, all consumers that compete for RES capacity are endowed with an amount of energy that is given by

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
\hspace{-30pt} && rse^{ES}_{\vartheta_i}(\mathbf{n}) = \min\left( E_{\vartheta_i}, \frac{\mathcal{ER}}{\sum_{\ell \in \Theta } n_{\ell }+1}\right),
\label{eq:eq_sharing_energy}
\end{eqnarray}
\normalsize
%where $n_0,n_1$ denote the number of competitors %of low-to-moderate and high energy profile \textit{but} player $i$, respectively, as also defined in Section 
%\ref{sec:prop_alloc}, and $n_0+n_1+1$ is the total number of competitors.
where $\sum_{\ell \in \Theta } n_{\ell }+1$ is the total number of competitors.%, with $n_0,n_1$ as in Section \ref{sec:prop_alloc}.

Generally, policies for sharing resources that accommodate a level of fairness that prioritizes classes of users with specific characteristics may provide high efficiency (by prioritizing ``strong players'') but lack stability (``weak players'' may continuously change behavior/strategy to improve the acquired service). For instance, the proportional allocation may cause unstable operational states since it entails the risk of starvation of users with low energy demand, and eventually result in fewer satisfied players. On the other hand, equal sharing of resources favors stability since it prevents strong energy players (consumers with high demand) from obtaining more resources that any other player. Yet, equal sharing may result in inefficient and wasteful utilization of energy resources, since the ``fair share'' of energy resources may exceed the energy requirements of particular consumers of low energy demand.

In the following sections, we analytically and numerically study the distributed, uncoordinated energy selection game. We study the stability and efficiency of energy resource allocation by considering the two different notions of fairness above. Specifically, for each allocation policy we analytically derive its equilibrium states (stability) and we numerically compare the costs incurred by the consumers' strategies against the costs of an optimal centralized coordinated operation (efficiency).

%
%enabling varying notions of fairness
%derive the stable operational states under the two allocation policies in terms of the associated equilibrium strategies, assuming fully rational players, free of knowledge and computational constraints.% and emotional biases.
%


% and analyze the resulting dynamics under different allocation policies that conceptualize various levels of fairness in energy resource sharing. In all cases, we derive the stable operational conditions (\ie equilibria) and the associated costs incurred by the players, and assess their efficiency by comparing them with those under optimal coordinated energy source allocation. 


\subsection{Demand}\label{sec:demand}
The expected aggregate demand for RES at NE, denoted as $D^{x,NE}$, is given as: %$N\sum_{\vartheta_j \in \Theta} r_{\vartheta_j }~p^{PA,NE}_{RES,\vartheta_j}~E_{\vartheta_j}$. % with respect to the energy profile 
\vspace{-5pt}
\footnotesize
\begin{eqnarray}
\hspace{-30pt} && D^{x,NE} (\mathbf{p^{x,NE}})= N\sum_{\ell\in \Theta} r_{\ell }~p^{x,NE}_{RES,\ell}~E_{\ell},
\label{eq:expected_demand}
\end{eqnarray}\normalsize where $x$ is replaced by $PA$ for the proportional allocation and by $ES$ for the equal sharing, and $p^{x,NE}_{RES,\vartheta_j}$ stands for the Nash equilibrium probability of profile $\vartheta_j \in \Theta$ competing for RES for each $x$ value. 

In Section, \ref{sec:uncoordinated_extra_demand}, we will give more explicit expressions for the expected aggregate demand dependent on the case.

\subsection{Social Cost}\label{sec:socialcost}
The social cost is computed differently for the proportional allocation and the equal sharing. In proportional allocation and at NE, 

\vspace{-5pt}
\footnotesize
\begin{align}
C^{PA,NE}(\mathbf{p}^{PA,NE}) &=  \min(\mathcal{ER}, D^{PA,NE}(\mathbf{p^{PA,NE}})) c_{RES} \nonumber \\&+  \max(0,D^{PA,NE}(\mathbf{p^{PA,NE}}))-\mathcal{ER})c_{nonRES,D} \nonumber \\
&+N \left[ \sum_{\ell \in \Theta} r_{\ell }p^{PA,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N}.
 \label{eq:social_cost_pa_extra_demand}
 \end{align}
\normalsize

For the equal sharing, we need to account for the extra renewable energy allocated to users, e.g., when all users (both profiles) compete for RES and possibly the lower energy profile users are allocated more RES than they need for or when the amount of RES is higher than the overall users' demand. The fair share of RES at NE, $sh(\mathbf{p^{ES,NE}})$, can be approximated by 

\vspace{-5pt}
\footnotesize
\begin{eqnarray}
sh(\mathbf{p^{ES,NE}}) \hspace{-5pt} &=& \hspace{-5pt} \frac{\mathcal{ER}}{ N \sum_{ \ell=0}^{M-1} r_{\ell}  E_{\ell} p_{RES,\ell}^{ES,NE}}.
 \label{eq:sharing_es}
 \end{eqnarray}
\normalsize

Therefore,
\vspace{-5pt}
\footnotesize
\begin{align}
&C^{ES,NE}(\mathbf{p^{ES,NE}}) \nonumber\\ &=  d(\mathbf{p^{ES,NE}}) c_{RES} +(D^{ES,NE} -d(\mathbf{p^{ES,NE}}))c_{nonRES,D}\nonumber \\
&+N \left[ \sum_{\ell\in \Theta} r_{\ell}p^{ES,NE}_{nonRES,\ell}\varepsilon_{\ell }E_{\ell}\right] c_{nonRES,N},
 \label{eq:social_cost_es}
 \end{align}
\normalsize

with \footnotesize$d(\mathbf{p^{ES,NE}})= N \sum_{ \ell=0}^{M-1} r_{\ell} p_{RES,\ell}^{ES,NE}  \min(sh(\mathbf{p^{ES,NE}}), E_{\ell})$.\normalsize


==> related.tex <==
\section{Related Work}\label{sec:related}

{Several works in the literature study DR as an essential mechanism of the smart grid for exploiting consumers' flexibility and providing services/benefits to the grid such as reducing costs of energy production/transmission/distribution and increasing the integration of the environmental friendly renewable energy without increasing the cost of reserves. Specifically, the consumers adapt their demand levels to the prices or other incentives that are appropriately determined by the utility companies, while both sides exchange information. A thorough review of different aspects (types, modeling, solution approaches, etc.) of DR mechanisms can be found in \cite{deng15,akbari2020concept}. Here, we indicatively briefly describe some of these works and emphasize on our contributions. In particular the problem studied in this paper relates to distributed DRPs with defferable loads.

In \cite{bitar17}, the authors introduce a DRP where consumers can reduce their energy procurement costs by requesting longer deadline periods, which provides flexibility to utility companies to satisfy demand. Contrary to our work, a centralized entity directly controls the deferrable loads so that the consumers' deadlines are respected and social welfare is maximized.
Furthermore, there is no differentiation in pricing when RES or conventional generation are used to satisfy the demand, but, only the deadline determines the relative price paid by the consumer.

Further works in the literature have studied distributed DRPs which indirectly incentivize consumers to shift their loads in response to price signals using game theoretic tools.
A dynamic pricing scheme is proposed in \cite{Caron10} to incentivize customers towards a load profile suitable for providers, highlighting the importance of information (load profiles) sharing to reduce cost overheads. In \cite{ibars2010distributed} a distributed load management is developed based on a non-cooperative game among consumers that controls the grid load at peak hours by means of dynamic pricing. In \cite{Joe_Wong12}, the authors formulate the electricity provider's cost minimization problem by considering consumers' device-specific scheduling flexibility and the provider's cost of purchasing electricity from an electricity generator.
%A novel appliance commitment algorithm that schedules thermostatically controlled household loads based on price and consumption forecasts is presented in \cite{DuLu11} seeking to minimize payments or maximize comfort.
Further works have focused on developing distributed control algorithms to achieve a Nash equilibrium in DRPs while preserving privacy and independence of the decision of the consumers. 
The paper \cite{jacquot18} thoroughly analyzes DR with an hourly billing scheme via a game theoretic viewpoint and proposes distributed algorithms to reach the Nash Equilibria while respecting users' privacy.
In \cite{stephens15}, multi-period DR in presence of storage is performed via Model Predictive Control (MPC) over a Nash non-cooperative game. Under perfect information, the unique Nash equilibrium strategies are Pareto optimal, otherwise unknown information may render the equlibria imperfect. The use of forecasts breaks the condition of perfect information but via MPC the Nash equilibria are re-computed with updated forecasts so as to be closer to Pareto optimality. A similar MPC approach over a non-cooperative game but without storage is proposed in  \cite{jacquot18}, where price forecasts are used. Contrary to our work, all these works do not study the choice of self-interested consumers over different energy sources with different prices, i.e., RES and conventional energy sources. Furthermore, in the aforementioned game theoretic modeling of distributed DRPs, the existence of a Nash equilibrium is shown but no closed-form solutions are obtained, and the performance of the Nash equilibrium with respect to centralized control is not studied.

In micro-grids, though non-cooperative game theoretic tools have been widely used to model DRPs, a gap remains in studying the loss of efficiency resulting from the self-interested behavior of consumers.
Indeed, Nash equilibrium in DRPs have been shown to be efficient for an infinite population EVs with identical charging rates \cite{ma2011decentralized}, and consumers without considering their utility curves \cite{}. However, these assumptions are impractical and quite restrictive.
In contract, in \cite{bai14}, the authors study the consumer energy consumption via a game theoretic model with a consumer utility function that trades-off its cost and convenience and study the differences with a system centralized approach that minimizes the aggregated energy cost.
%%%%%%
In \cite{jia16}, the authors compare the centralized or decentralized ownership and control of RESs and storage using Stackelberg game models. They trade-off cost and consumers' convenience and conclude that a centrally owned (by an operator) integration brings more benefits for both consumers and utilities. Yet, no bounds on the PoA is derived in these papers. The authors in \cite{rodriguez2021value} compute the PoA over a non-cooperative game of consumers and show that this loss of efficiency is mainly related to the centralization of information.
Similarly, the authors in \cite{chakraborty2017distributed} study the distributed control of loads using a PA policy. In this work, the central coordinator aims at setting the optimal price which incentivizes consumers to adapt their load profiles based on renewable energy production forecasts in the intra-day. A game-theoretic analysis of this mechanism shows the existence of a Nash equilibrium both for price-taker consumers and price-anticipator consumers, and derive a bound on the PoA of this DRP. Yet, in the aforementioned papers, contrary to our work, competition over multiple energy sources and differences in risk attitudes of consumers are not accounted for.
%%%%

%In \cite{mohsenian2010autonomous} the authors present an incentive-based energy consumption scheduling game among consumers with a single utility company and show that the global optimization of energy costs is achieved at Nash equilibrium. 

%%%%


  % The management of demand required by storage energy devices is addressed in \cite{vytelingum2010agent}, where the authors provide a generic framework to analyze the Nash equilibrium of an electricity grid and devise agent-based storage learning strategies %that adapt to market conditions reducing 
%to reduce the peak demand, costs and carbon emissions. 

%The development of the open energy market along with the integration of RES in the grid has led to several studies of DR assuming the existence of multiple utilities \cite{chai14}, \cite{maharjan13}, \cite{maharjan16}. Indeed, consumers also choose utility company to buy power for their demands, and therefore, utilities become selfish rational competitors. Such interactions are studied using hierarchical games, i.e., the Stackelberg Game Approach. The utility companies at the top level of the hierarchy play a non-cooperative game \cite{chai14}, \cite{maharjan13} and the consumers at the lower level respond optimally to the utilities' strategies and studied via evolutionary game theory \cite{chai14}. 


Our work focuses on competition with respect to choosing energy sources and differs from related works that mainly focus on competition across time for the capacity of a single energy provider (incorporating many energy sources as a single entity) dealing with scheduling shiftable demand loads (\hspace{0.5pt}\cite{Joe_Wong12}, %\cite{Rooz10}, 
\cite{Caron10}, \cite{ibars2010distributed}, %\cite{li2011optimal}, 
 \cite{DuLu11}). %, \cite{mohsenian2010autonomous}). %In addition, contrary to \cite{bu2011stochastic}, \cite{he2011multiple}, we investigate optimization of both individual (power consumption) and aggregate (power generation) cost.
Furthermore, we consider a multi-energy context in line with \cite{maharjanuser}, yet we differentiate consumers in terms of both their demand and their risk-attitude, allowing also different levels of fairness in the energy allocation. Most importantly, we draw a generic analytical framework relative to settings with variant references to cost and energy units.}




==> related_work/v2_intro/brief/introduction.tex <==
\section{Introduction}\label{sec:intro}

One of the key features of the SG is the replacement of conventional mechanical meters with smart meters to enable efficient, flexible and reliable two-way flow of energy and information for better coordination between suppliers and customers and control of the power grids. Renewable energy sources (RES), e.g. wind turbines and solar photovoltaics, have become one of the critical parts in SG, as well as more and more users are willing to deploy the RES and energy storage devices at their homes \cite{farmad2012integration}. This paper explores an approach to utilize the maximum available of RES taking into consideration the recognized problem of carbon pollution. By 2020, it is expected that almost 72\% of European consumers will have a smart electric meter.

Demand response management (DRM) smooths out the system power demand profile across time and provides short-term reliability benefits as it can offer load relief to resolve system and/or local capacity constraints. Thus, from the operator aspect, DRM reduces the cost of operating the grid, while from the user aspect it lowers their bills. In most of the past papers that have modeled renewable energy (RE), e.g \cite{bu2011stochastic}, \cite{he2011multiple}, the key focus has been on exploring DRM in the context of multiple energy sources, incorporating RESs on the supply side and minimizing the cost of this side. Instead, \cite{maharjanuser} includes multiple renewable and non-renewable energy sources based utility companies and focuses on minimizing the cost for each user.
Recently, game theory has been applied to the Demand Response programs \cite{saad2012game}. For example, the non-cooperative game was utilized to minimize the electricity cost of consumers \cite{mohsenian2010autonomous}, where based on a common scenario, with a single utility company serving multiple customers, the global optimal performance in terms of minimizing the energy costs is achieved at the Nash equilibrium of the formulated energy consumption scheduling game

Most of the demand-side management (DSM) approaches that have been deployed over the past three decades (e.g. \cite{ruiz2009direct}), focus on the interactions between a utility company (UC) and its customers or users. In contrast, Mohsedian-Rad et al. \cite{mohsenian2010autonomous} argue that rather than focusing on how each user behaves individually, a good DSM program should have the objective that the aggregate load satisfies some desired properties. More specifically, this work presents an incentive-based energy consumption scheduling scheme, where through an appropriate pricing scheme, the Nash equilibrium of the energy consumption game among the participating users who share the same energy source is the optimal solution that minimizes the energy cost in the system.

However, in the future SGs, energy storage is expected to be a key component in smart homes and thus, it has a strong impact on DSM. In \cite{vytelingum2010agent}, Vytelingum et al. provide a general framework within which to analyze the Nash equilibrium of an electricity grid and devise new agent-based storage learning strategies that adapt to market conditions. The simulation results show that the learning scheme converges to a Nash equilibrium while reducing the peak demand which also leads to reduce costs and carbon emissions. Based on the normal electricity usage profile of all the users in the considered SG, it is then possible to compute the Nash equilibrium points, which describe when it is best for the agents to charge their batteries, use their stored electricity, or use electricity from the SG \cite{fadlullah2011survey}.

Storage devices may be used to compensate for the variability of typical renewable electricity generation including wind, wave and solar energy. With this motivation, \cite{maharjanuser} includes multiple renewable energy sources on the supply side, in addition to the traditional fossil-fuel based sources. In \cite{mohsenian2010autonomous}, \cite{ibars2010distributed}, \cite{jia2012optimal} users are price anticipating (i.e., they take into account how their consumptions will affect the prices). For example, in \cite{ibars2010distributed} is defined a non-cooperative congestion game among users, which is used to set the price levels for the demand vector of each user. On the contrary, in case where users are price taking (\cite{li2011optimal},\cite{yang2013game}), they aim to minimize their costs.

There has been a growing interest in last years in modeling ICT systems and applications where a number of selfish agents compete over a limited capacity and low-cost resource. Very recent work, \cite{hasan2012non} and \cite{shi2011competition} has been focused on addressing the competition in game-theoretic terms. With the same spirit, in \cite{holzman2003network}, the drivers choose between a number of routes from a common-to-all origin to a common-to-all destination. In a nutshell, all the works noted above, apply selection games where players choose between specific available resources. In contrast, in this paper we consider the choice between specific sources at any time period. In our uncoordinated source selection problem, consumers are viewed as strategic decision-makers that aim at maximizing their own individual welfare.






==> related_work/v2_intro/extended/introduction.tex <==
\section{Introduction}\label{sec:intro}

Recently, the Smart Grid (SG) has been proposed as the next-generation architecture of electrical grid that modernizes the current power grids for better utilization of existing assets. One of the key features of the SG is the replacement of conventional mechanical meters with smart meters to enable efficient, flexible and reliable two-way flow of energy and information for better coordination between suppliers and customers and control of the power grids. Renewable energy sources (RES), e.g. wind turbines and solar photovoltaics, have become one of the critical parts in SG, as well as more and more users are willing to deploy the RES and energy storage devices at their homes \cite{farmad2012integration}. This paper explores an approach to utilize the maximum available of RES taking into consideration the recognized problem of carbon pollution.
Based on a report of the European Wind Energy Association, in 2013 EU member states had an installed wind generation capacity of 117,289MW. This is expected to increase to meet the EU Commission's sustainability target, which is that 27\% of generation must come from renewable sources by 2030. Germany is leading the world in the development and implementation of photovoltaic solar power. Japan has similarly moved to the forefront of distribution automation through its use of advanced battery-storage technology. Totally, EU member states have committed to rolling out close to 200 million smart electric meters. By 2020, it is expected that almost 72\% of European consumers will have a smart electric meter. These smart meters can be used not only to provide more accurate billing for customers but can also be leveraged by distribution network operators for improved outage management processes, power quality and demand response programs, each of which will allow for increased network reliability.

Demand Response (DR) is the response system of the end-users to manage their consumption of electricity in response to supply conditions. Demand response management (DRM) smooths out the system power demand profile across time and provides short-term reliability benefits as it can offer load relief to resolve system and/or local capacity constraints. Thus, from the operator aspect, DRM reduces the cost of operating the grid, while from the user aspect it lowers their bills. In most of the past papers that have modeled renewable energy (RE), e.g \cite{bu2011stochastic}, \cite{he2011multiple}, the key focus has been on exploring DRM in the context of multiple energy sources, incorporating RESs on the supply side and minimizing the cost of this side. Instead, \cite{maharjanuser} includes multiple renewable and non-renewable energy sources based utility companies and focuses on minimizing the cost for each user.
Recently, game theory has been applied to the DR programs \cite{saad2012game}. For example, the non-cooperative game was utilized to minimize the electricity cost of consumers \cite{mohsenian2010autonomous} and the congestion game was applied to control the electricity consumption by dynamic pricing \cite{ibars2010distributed}. The research work in \cite{mohsenian2010autonomous} formulates an energy consumption scheduling game, where the players are the users and their strategies are the daily schedules of their household appliances and loads. Based on a common scenario, with a single utility company serving multiple customers, the global optimal performance in terms of minimizing the energy costs is achieved at the Nash equilibrium of the formulated energy consumption scheduling game.

Most of the demand-side management (DSM) approaches that have been deployed over the past three decades (e.g. \cite{ruiz2009direct}), focus on the interactions between a utility company (UC) and its customers or users (via Real-Time Pricing, Direct Load Control, etc.), that reveal users' privacy problems when it comes to residential load control and home automation. In contrast, Mohsedian-Rad et al. \cite{mohsenian2010autonomous} argue that rather than focusing on how each user behaves individually, a good DSM program should have the objective that the aggregate load satisfies some desired properties. More specifically, this work presents an incentive-based energy consumption scheduling scheme, where through an appropriate pricing scheme, the Nash equilibrium of the energy consumption game among the participating users who share the same energy source is the optimal solution that minimizes the energy cost in the system. The experimental results reveal that this approach is able to reduce the peak-to-average ratio of the total energy demand, the total energy costs, and also each user's individual daily electricity bills.
The previous work was focused on how the users can schedule their appliances so as to minimize their billing charges. The underlying assumption was that the users are acquiring energy so as to immediately use it for their appliances.

However, in the future SGs, energy storage is expected to be a key component in smart homes and thus, it has a strong impact on DSM. In \cite{vytelingum2010agent}, Vytelingum et al. provide a general framework within which to analyze the Nash equilibrium of an electricity grid and devise new agent-based storage learning strategies that adapt to market conditions. The simulation results show that the learning scheme converges to a Nash equilibrium while reducing the peak demand which also leads to reduce costs and carbon emissions. Based on the normal electricity usage profile of all the users in the considered SG, it is then possible to compute the Nash equilibrium points, which describe when it is best for the agents to charge their batteries, use their stored electricity, or use electricity from the SG \cite{fadlullah2011survey}.

Storage devices may be used to compensate for the variability of typical renewable electricity generation including wind, wave and solar energy. With this motivation, \cite{maharjanuser} includes multiple renewable energy sources on the supply side, in addition to the traditional fossil-fuel based sources. Specifically, the users schedule their demands by optimally choosing the UCs and by optimally scheduling their shiftable appliances in order to minimize their payments to the providers. They formulate the problem as a game, incorporating the uncertainty associated with the power supply of the renewable sources, and prove that there exists a Nash equilibrium for the game.

In \cite{mohsenian2010autonomous}, \cite{ibars2010distributed}, \cite{jia2012optimal} users are price anticipating (i.e., they take into account how their consumptions will affect the prices). For example, in \cite{ibars2010distributed} is defined a non-cooperative congestion game among users, which is used to set the price levels for the demand vector of each user. The work demonstrates that the game formulated as such converges to a stable equilibrium point in a distributed manner. Furthermore, the work not only finds the local optimum points of the Nash equilibria but also shows that it is possible to arrive at a global solution to the network problem by using the equivalence between the congestion and potential games. On the contrary, in case where users are price taking (\cite{li2011optimal},\cite{yang2013game}), they aim to minimize their costs.

There has been a growing interest in last years in modeling ICT systems and applications where a number of selfish agents compete over a limited capacity and low-cost resource. Very recent work, \cite{hasan2012non} and \cite{shi2011competition} has been focused on addressing the competition in game-theoretic terms. With the same spirit, in \cite{holzman2003network}, the drivers choose between a number of routes from a common-to-all origin to a common-to-all destination. Likewise, in an instance of the access-point association problem, a number of mobiles compete over a finite number of access points where high access delays occur when many users associate with the same wireless access point \cite{hasan2012non}. In a nutshell, all the works noted above, apply selection games where players choose between specific available resources. In contrast, in this paper we consider the choice between specific sources at any time period. In our uncoordinated source selection problem, consumers are viewed as strategic decision-makers that aim at maximizing their own individual welfare.






==> uncoordinated.tex <==
\vspace{-0.05in}
\section{Game analysis} \label{sec:analysis}
\vspace{-0.05in}
%\subsection{Existence of NE}
Here, we study the conditions on the parameter values for the existence of dominant strategies and NE under PA.

%The defined Energy Source Selection Game is finite and thus it has \textit{at least} one mixed strategy NE.
To derive the NE, we recall that any mixed strategy equilibrium $\mathbf{p^{NE}}$
%=(\mathbf{p_0^{NE}}, \mathbf{p_1^{NE}}, ..., \mathbf{p_{M-1}^{NE}})^T$, with $\mathbf{p}^{NE}_{\ell}=[p^{NE}_{RES,\ell}, p^{NE}_{nonRES,\ell}]^T$, 
must fulfill

\vspace{-0.08in}
\small
\begin{equation}\label{eq:cost_equality_mixed}
\upsilon_{RES, \ell}(\mathbf{p^{NE}})= \upsilon_{nonRES, \ell}(\mathbf{p^{NE}}), ~\forall \ell \in \Theta.
\end{equation}
\normalsize
Namely, the expected costs of each pure strategy in the support of the equilibrium mixed strategy ($\mathcal{A}$) are equal. By replacing in \eqref{eq:cost_equality_mixed} the expressions of \eqref{eq:RES_cost} and \eqref{eq:nonRES_cost2}, we obtain that at a NE the amount of RESs allocated to $\ell \in \Theta$ should satisfy

\vspace{-0.08in}
\small
\begin{equation}\label{eq:conditionEQ_extra_demand}
rse^{PA, NE}_{\ell}(\mathbf{p^{NE}}) = \frac{\gamma-\epsilon_{\ell}\beta}{\gamma-1}E_{\ell},~ \forall \ell \in \Theta.
\end{equation}
\normalsize
%\subsection{Close-form expression of NE}
Thus, when combining the Energy Source Selection Game with the PA policy, the existence of a NE is under the condition

\vspace{-0.08in}
\small
\begin{equation}\label{eq:condition_PA_NE}
rse_{\ell}^{PA}(\mathbf{p}^{NE}) =rse_{\ell}^{PA,NE}(\mathbf{p}^{NE}), \forall \ell \in \Theta. \end{equation}
\normalsize
Next we give the conditions such that either \eqref{eq:condition_PA_NE} holds and mixed NE exist or there exist dominant strategies. For this study, we distinguish cases with respect to the RES capacity, the risk aversion degree values and the day-time energy demand levels. 

\begin{remark}
For all cases, any existing NE competing probabilities, $\mathbf{p}^{NE}$, are obtained so as to satisfy the relation \eqref{eq:condition_PA_NE}.\end{remark}

\subsubsection{Case $1$} \emph{The RES capacity, $\mathcal{ER}$, exceeds the quantity $D^{Total}$.} As the consumers have knowledge of $\mathcal{ER}$ and $D^{Total}$, it is straightforward to show that the dominant strategy for all consumers is to play $RES$ and the aggregate demand for RESs is equal to $D^{Total}$.

In all the remaining cases, we assume that $\mathcal{ER}< D^{Total}$. %These three distinct cases are defined with respect to the risk aversion of the consumers.

\subsubsection{Case $2$} \emph{The risk aversion degrees for all consumers' types satisfy $1\leq \epsilon_{\ell}<\gamma/\beta$, $\forall \ell \in \Theta$.}
We distinguish the following sub-cases with respect to the day-time energy demand levels. 

\textbf{Sub-case $2(a)$:} 
\emph{The day-time energy demand levels satisfy  $E_{\ell } \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell }\beta)}$,  for all $\ell \in \Theta$.} Then, a mixed-strategy NE with the PA policy exists if and only if for every pair of consumers, $i,j$ with day-time energy demand levels $E_{\vartheta_i}$, $E_{\vartheta_j}$, respectively, it holds that

\vspace{-0.1in}
\small
\begin{eqnarray}\label{eq:relation_E_0_E_1_pa_ne_extra_demand}
\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i }\beta)}-E_{\vartheta_i} &=& \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j }\beta)}-E_{\vartheta_j}.
 \end{eqnarray}
\normalsize

To derive the condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} we first re-write \eqref{eq:condition_PA_NE} assuming that consumer $i$ with type $\vartheta_i \in \Theta$ plays $RES$ (in \eqref{eq:probrelation1}) and then similarly for $\vartheta_j \in \Theta \setminus \{\vartheta_i\}$ (in \eqref{eq:probrelation2}), as follows:

\vspace{-0.1in}
\begin{small}
\begin{align}
&  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i}= \sum_{ {\ell}\in \Theta} r_{\ell}~ (N-1)~E_{\ell}~p^{NE}_{RES,\ell},
    \label{eq:probrelation1}\\
  &  \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_j}\beta)}-E_{\vartheta_j}=  \sum_{ {\ell}\in \Theta} r_{\ell} ~(N-1)~E_{\ell}~ p^{NE}_{RES,\ell}.
    \label{eq:probrelation2}  
\end{align}
\end{small}
%Eq. \eqref{eq:condition_PA_NE} can be re-written in a similar way for any other type $\vartheta_j \in \Theta$. 
Note that to derive (\ref{eq:probrelation1}) we consider that if consumer $i$ plays $RES$, then, $D(\mathbf{p^{NE}})$ can be expressed as $E_{\vartheta_i}+ \sum_{ {\ell}\in \Theta} r_{\ell}~ (N-1)~E_{\ell}~p^{NE}_{RES,\ell}$ for a large number of consumers. Similarly for (\ref{eq:probrelation2}). Then, since the right-hand sides of \eqref{eq:probrelation1}-\eqref{eq:probrelation2} are equal, the left-hand sides will be also equal and \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} derives. %\eqref{eq:probrelation1}-\eqref{eq:probrelation2} 
Furthermore, at NE, the expected aggregate demand for RES can be expressed, for any $\ell \in \Theta$, as:

\footnotesize
\begin{align}
& D(\mathbf{p}^{NE})= \min\Bigl\{D^{Total}, \max\Bigl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}-E_{\ell}\right]\frac{N}{(N-1)},0\Bigr\}\Bigr\}.
    \label{eq:demand1}
\end{align}
\normalsize

To construct \eqref{eq:demand1}, we multiplied \eqref{eq:probrelation1} with $\frac{N}{N-1}$ and used the definition of the demand for RESs in \eqref{eq:demand}.

\begin{remark}\label{rem:risk_seeking}If all consumers are risk-seeking (i.e., $\epsilon_{\vartheta_i}= 1, \forall i \in \mathcal{N}$), a NE can exist only if  $E_{0}=E_{1}=...=E_{M-1}$.%for every pair of $\vartheta_i, \vartheta_j \in \Theta$. %On the contrary, if there are risk-conservative consumers, they may need to have asymmetric energy profiles for a NE to exist.
\end{remark}

\begin{remark} \label{rem:risk_degrees_relation}
Note that condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand} can hold, and therefore a NE can exist, only if $\epsilon_0\leq \epsilon_1 \leq..\leq \epsilon_{M-1}$. Since by assumption, $E_0\leq E_1 \leq ...\leq E_{M-1}$, this means that consumers with lower day-time energy demand levels should be less risk-averse than those with higher ones.
\end{remark}

 
\textbf{Sub-case $2(b)$:} 
\emph{The day-time energy demand levels satisfy $E_{\ell} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}$  for all $\ell \in \Theta$.} In this case, the dominant strategy for all consumers is to play $nonRES$ and cover their entire energy profiles ($U_{\ell}$) at night.

To prove this, we show that $\upsilon_{RES, \vartheta_i}(\mathbf{p})>\upsilon_{nonRES, \vartheta_i}(\mathbf{p})$, $\forall \mathbf{p}$ and $\forall i\in \mathcal{N}$. Assume that $\vartheta_i=0$ and that the allocated energy is $E'$. Then, we have that $\upsilon_{RES, 0}(\mathbf{p})= E'  \cdot c_{RES}+(E_0-E')\cdot \gamma \cdot  c_{RES}$ and 
$\upsilon_{nonRES, 0}(\mathbf{p})= \epsilon_0 \cdot E_0 \cdot \beta \cdot c_{RES}$. The inequality $\upsilon_{RES,0}(\mathbf{p})>\upsilon_{nonRES, 0}(\mathbf{p})$ is then equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$, which is true by assumption, since $E'<\mathcal{ER}$. Similar proofs hold for every type $\ell \in \Theta$.


\textbf{Sub-case $2(c)$:}
\emph{There exist two distinct subsets of consumers' types, $\Sigma_1 , \Sigma_2 \subset \Theta$, where $\{E_{\ell} > \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}, ~\forall \ell \in \Sigma_1\}$ and $\{E_{\ell} \leq \mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}, ~ \forall \ell \in \Sigma_2\}$.} For consumers in the set $\Sigma_1$, the dominant strategy is to play $nonRES$ and to cover their entire energy profiles ($U_{\ell}$) during the night. The explanation is the same as in Sub-case $2(b)$.
For consumers in the set $\Sigma_2$, the mixed strategy NE is determined under the condition of \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}. Remark \ref{rem:risk_degrees_relation} holds for all types in $\Sigma_2$, and the expected aggregate demand for RESs can be expressed by analogy with \eqref{eq:demand1}, in which $D^{Total}$ is replaced by the maximum expected total demand for RESs of the consumers whose types are in $\Sigma_2$, i.e., $D^{Total}_{\Sigma_2} = N  \sum_{\tilde{\ell } \in \Sigma_2} r_{\tilde{\ell }  }E_{\tilde{\ell } }$.

%\vspace{-5pt}
%\footnotesize
%\begin{align}
%&D(\mathbf{p}^{NE})= \min\Biggl \{N  \sum_{\tilde{\ell } \in \Sigma_2} r_{\tilde{\ell }  }E_{\tilde{\ell } }, \max\Biggl\{\left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{\ell}\beta)}-E_{\ell}\right]\nonumber\\ & .\frac{N}{(N-1)},0\Biggr\}\Biggr\}.
 %   \label{eq:demand2}
%\end{align}
%\normalsize

%\begin{remark}
%In the special case of two consumers, one in $\Sigma_1$ (with index $1$) and the other in $\Sigma_2$ (with index $0$), we obtain 
%$p^{NE}_{RES,0}  =\min \left\{1, \max \left\{0, \left[\mathcal{ER}\frac{(\gamma-1)}{(\gamma-\epsilon_{0}\beta)}-E_{0}\right]\frac{1}{r_{0}(N-1)E_{0}}\right\}\right\}$.
%\end{remark}
%\vspace{1pt}

\subsubsection{Case $3$} \emph{The risk aversion degrees satisfy $\epsilon_{\ell} \geq \gamma/\beta$, $\forall \ell \in \Theta$.} In this case, the dominant strategy for all consumers is to play $RES$. To show this, assume that $\ell=0$ and that the allocated energy is $E'$. Then, the inequality $\upsilon_{RES,0}(\mathbf{p})<\upsilon_{nonRES, 0}(\mathbf{p})$ is equivalent to the inequality $E_0 >E' \frac{(\gamma-1)}{(\gamma-\epsilon_0\beta)}$. This is true by assumption, since $(\gamma-\epsilon_0\beta)\leq 0$ in this case. 

\subsubsection{Case $4$} \emph{There exist two distinct subsets of consumers' types, $\Sigma_1$, $\Sigma_2 \subset \Theta$, where $\Bigl\{\epsilon_{\ell} \geq \gamma/\beta, ~ \forall \ell \in \Sigma_1\Bigr\}$, and $\Bigl\{\epsilon_{\ell} < \gamma/\beta,~\forall \ell \in \Sigma_2\Bigr\}$.} For consumers in the set $\Sigma_1$, the dominant strategy is to compete for RESs, which is shown by analogy with Case $3$.
For consumers in the set $\Sigma_2$, the conditions derived in Case $2$ can straightforwardly be extended to the consumer types in $\Sigma_2$, considering that all consumers in $\Sigma_1$ play $RES$. To do so, we consider that the available RES capacity for consumers in $\Sigma_2$ is equal to $\mathcal{ER}$ minus the aggregate demand for RESs of consumer types in $\Sigma_1$. For the sake of concision we do not detail these conditions.


%is determined under condition \eqref{eq:relation_E_0_E_1_pa_ne_extra_demand}. Remark \ref{rem:risk_degrees_relation} holds for all consumers in $\Sigma_2$.
%In addition, the expected aggregate demand for RESs at NE can be expressed for any consumer $i \in \mathcal{N}$, as

%\footnotesize
%\begin{align}
%& D(\mathbf{p}^{NE})= N  \sum_{\ell \in \Sigma_1} r_{\ell }E_{\ell}+\min\Biggl\{N  \sum_{\ell \in \Sigma_2} r_{\ell }E_{\ell}, \max\Biggl\{  \Bigl[\mathcal{ER}\nonumber \\  & \cdot \frac{(\gamma-1)}{(\gamma-\epsilon_{\vartheta_i}\beta)}-E_{\vartheta_i} -\sum_{\ell \in \Sigma_1 \setminus \{\vartheta_i \}} r_{\ell} (N-1)E_{\ell}\Bigr]\frac{N}{(N-1)},0\Biggr\}\Biggr\}.
 %   \label{eq:demand3}
%\end{align}
%\normalsize


